Absolute Expressiveness of Subgraph-based Centrality Measures

In graph-based applications, a common task is to pinpoint the most important or ``central'' vertex in a (directed or undirected) graph, or rank the vertices of a graph according to their importance. To this end, a plethora of so-called centrality measures have been proposed in the literature. Such measures assess which vertices in a graph are the most important ones by analyzing the structure of the underlying graph. A family of centrality measures that are suited for graph databases has been recently proposed by relying on the following simple principle: the importance of a vertex in a graph is relative to the number of ``relevant'' connected subgraphs surrounding it; we refer to the members of this family as subgraph-based centrality measures. Although it has been shown that such measures enjoy several favourable properties, their absolute expressiveness remains largely unexplored. The goal of this work is to precisely characterize the absolute expressiveness of the family of subgraph-based centrality measures by considering both directed and undirected graphs. To this end, we characterize when an arbitrary centrality measure is a subgraph-based one, or a subgraph-based measure relative to the induced ranking. These characterizations provide us with technical tools that allow us to determine whether well-established centrality measures are subgraph-based. Such a classification, apart from being interesting in its own right, gives useful insights on the structural similarities and differences among existing centrality measures.

==> app-directed.tex <==
\subsection*{Preliminaries}
%

A {\em directed graph} (or {\em digraph} for short) $G$ is a pair $(V,E)$, where $V$ is a finite non-empty subset of $\ins{V}$ (the set of {\em vertices of $G$}), and $E \subseteq \{(u,v) \mid u,v \in V\}$ (the set of {\em edges of $G$}). As for undirected graphs, we write $V(G)$ and $E(G)$ for the set of vertices and edges of $G$, respectively.
%
A {\em multi-graph} $M$ is defined in the same way as undirected graphs, with the key difference that the edges from a multiset (or a bag), i.e., we can have more than one undirected edges between two vertices.
%
The notations $V(M)$ and $E(M)$ can ba naturally defined for multi-graphs.
%
Given a directed graph $G$, the undirected version of it, denoted $\text{UN}(G)$, is defined as the multi-graph $(V(G),[\{u,v\} \mid (u,v)\in E(G) \text{ or } (v,u)\in E(G)])$. 
%
Note that we use the notation $[\cdot]$ to denote bags. For example, $[a,a,b]$ is the bag consisting of two occurrences of $a$ and one occurrence of $b$.
%
We say that a directed graph $G$ is connected if the multi-graph $\text{UN}(G)$ is connected. This notion of connectedness is known in the literature as weak connectedness. In simple words, $G$ is connected if the multi-graph obtained after removing the directions of the edges is connected.
%
For a vertex $v$ in a directed graph $G$, we define the children of $v$ in $G$ as the set $\text{OUT}(v,G) = \{u\in V(G) \mid (v,u)\in E(G)\}$ and the parents of $v$ in $G$ as the set $\text{IN}(v,G) = \{u\in V(G)\mid (u,v)\in E(G)\}$.
%
A connected subgraph of $G$ is any graph $G'$ such that $V(G')\subseteq V(G)$ and $E(G')\subseteq E(G) \cap (V(G')\times V(G'))$, and we write $G'\subseteq G$ to indicate that $G'$ is a subgraph of $G$.
%
Given a vertex $v \in V(G)$, we define the set of all connected subgraphs containing $v$ in $G$ as $\A(v,G) = \{G' \subseteq G\mid v\in V(G') \text{ and } G' \text{ is connected}\}$. Given two vertices $u,v$ in $V(G)$, a path connecting $u$ and $v$ is a sequence of vertices $\pi_{uv} = w_1w_2...w_n$ such that $w_1 = u$, $w_n=v$ and, for every $i\in\{1,..,n-1\}$, $(w_i,w_{i+1})\in E(G)$. The size of $\pi_{uv}$ is defined as $|\pi_{uv}| = n-1$. By convention, $\pi_{uu} = u$ and $|\pi_{uu}| = 0$. 
%
A {\em connected component} (or simply {\em component}) of $G$ is an induced subgraph $G[S]$ of $G$, where $S \subseteq V(G)$, such that $G[S]$ is connected, and, for every $v \in V(G) \setminus S$, there is no path in $G$ from $v$ to a vertex of $S$ neither a path from any vertex in $S$ to $v$. We denote by $\comp(G)$ all the components of $G$, that is, the set of graphs $\{G' \mid G' \text{ is a component of } G\}$. We define the reachable component of a node $v$ in $G$ as the set $K_{v}(G)\subseteq V(G)$ such that $K_{v}(G)=\{u\in V(G)\mid \text{there exists a path from $v$ to $u$ in } G\}$.
%
We denote by $\gr$ the set of all digraphs, and by $\vg$ the set of vertex-digraph pairs $\{(v,G) \in \ins{V} \times \gr \mid v \in V(G)\}$. Note that we overload the notation and we use $\gr$ and $\vg$, as for undirected graphs, to refer to the set of all digraphs and the set of vertex-digraph pairs, respectively. This will not cause any confusion as the rest of the appendix is only about digraphs.
%
Note that two digraphs $G_1$ and $G_2$ are {\em isomorphic}, denoted $G_1\simeq G_2$, if there exists a bijective function $h: V(G_1) \to V(G_2)$ such that $(v,u) \in E(G_1)$ iff $(h(v),h(u))\in E(G_2)$.
%
Furthermore, given the vertices $v_1 \in V(G_1)$ and $v_2 \in V(G_2)$, we say that the pairs $(v_1, G_1)$ and $(v_2,G_2)$ are isomorphic, denoted $(v_1, G_1) \simeq (v_2,G_2)$, if $G_1\simeq G_2$ witnessed by $h$, and $h(v_1)= v_2$.
%
A centrality measure for digraphs is defined in the same way as for undirected graphs, i.e., as a function from $\vg$ to $\mathbb{R}$ that is closed under isomorphism.
%

In the rest of the appendix, we may say graph meaning digraph, and we only refer to measures for digraphs.

 %In the case of directed graphs, for $n>0$, we denote the line graph as $L_n:=(\{1,...,n\},\{(i,i+1)\mid i\in\{1,...,n-1\})$. We denote the star graph, in the other hand, as the graph $S_n = \{\{1,...,n\},\{(i,1)\mid i\in\{2,...,n\}\}$.

\subsection*{Special Graphs}
%

The {\em line graph} with $m>0$ vertices, denoted $L_m$, is the digraph $(V,E)$, where 
\[
V\ =\ \{1,\ldots,m\} \quad \text{and} \quad E = \bigcup_{i \in \{1,\ldots,m-1\}}\{(i,i+1)\}.
\]


\noindent The {\em star graph} with $m>0$ vertices, denoted $S_m$, is the digraph $(V,E)$, where
\[
V\ =\ \{1,\ldots,m\} \quad \text{and} \quad E\ =\ \bigcup_{i \in \{2,\ldots,m\}} \{(i,1)\}.
\]
We refer to the vertex $1$ as the center of $S_m$.

\begin{comment}
\subsection*{Closure Under Isomorphism}
%

We say that two digraphs $G_1$ and $G_2$ are {\em isomorphic}, denoted $G_1\simeq G_2$, if there exists a bijective function $h: V(G_1) \to V(G_2)$ such that $(v,u) \in E(G_1)$ iff $(h(v),h(u))\in E(G_2)$.
%
Furthermore, given the vertices $v_1 \in V(G_1)$ and $v_2 \in V(G_2)$, we say that the pairs $(v_1, G_1)$ and $(v_2,G_2)$ are isomorphic, denoted $(v_1, G_1) \simeq (v_2,G_2)$, if $G_1\simeq G_2$ witnessed by $h$, and $h(v_1)= v_2$.
%
We are now ready to define the property of being closed under isomorphism for centrality measures.


\begin{definition}\label{def:closed-under-iso-directed}
	Consider a centrality measure $\Ce$. We say that $\Ce$ is {\em closed under isomorphism} if, for every two pairs $(v_1,G_1) \in \vg$ and $(v_2,G_2) \in \vg$, $(v_1, G_1) \simeq (v_2,G_2)$ implies $\Ce(v_1,G_1) = \Ce(v_2,G_2)$. \hfill\markfull
\end{definition}


In simple words, the above property states that the values assigned by a measure to the vertices of a graph do not depend on the names of the vertices, but only on the structure of the graph; hence, the above property is sometimes called {\em anonymity}.
\end{comment}

\subsection*{Locality}
%

We finally recall the so-called locality property. Recall that, given a graph $G$ and a set of vertices $S \subseteq V(G)$, we write $G[S]$ for the subgraph of $G$ induced by $S$.
%
The definition of locality follows:

\begin{definition}\label{def:locality-directed}
	A centrality measure $\Ce$ is {\em local} if, for every pair $(v,G) \in \vg$, $\Ce(v,G) = \Ce(v,G[K_v(G)])$. \hfill\markfull
\end{definition}


In simple words, the above property tells us that the value assigned by a measure $\Ce$ to a vertex $v$ in a graph $G$ depends only on the component $G' \in \comp(G)$ that contains $v$, i.e., during the calculation of $\Ce(v,G)$, $\Ce$ considers only the component $G'$.


\subsection*{Subgraph Motif Measures for Directed Graphs}

We proceed to introduce the family of subgraph motif measures for directed graphs. This is actually done in the exactly the same way as for undirected graphs. Nevertheless, for the sake of completeness and clarity, we give here all the definitions.
%
A {\em subgraph family} is a function $\mathsf{F}: \vg \to \mathcal{P}(\gr)$ such that:

\begin{itemize}
	\item  for every pair $(v,G)\in \vg$, $\mathsf{F}(v,G) \subseteq \A(v,G)$.
	
	\item for every two pairs $(v_1,G_1) \in \vg$ and $(v_2,G_2) \in \vg$ such that $(v_1,G_1) \simeq (v_2,G_2)$ witnessed by $h$, there exists a bijection $\mu : \F(v_1,G_1) \rightarrow \F(v_2,G_2)$ such that, for every $G' \in \F(v_1,G_1)$, $\mu(G') = (\{h(v) \mid v \in V(G')\},\{(h(v),h(u)) \mid (v,u) \in G'\})$.
\end{itemize}  

\noindent A filtering function is a function $f:\mathbb{N}\to\mathbb{R}$. 


\begin{definition}[\textbf{Subgraph Motif Measure (for Directed Graphs)}]\label{def:subc-digraphs}
	Consider a subgraph family $\F$ and a filtering function $f$. The {\em $\langle \F,f \rangle$-measure} is the function 
	$
	\subc{\F,f} : \vg\ \rightarrow\ \mathbb{R}
	$
	such that, for $(v,G) \in \vg$, $\subc{\F,f}(v,G) = f(|\F(v,G)|)$.
\end{definition}
	%
	
	Since, by definition, subgraph families are closed under isomorphism, it is straightforward to see that each $\langle \F,f \rangle$-measure defines a valid centrality measure.
	
	\begin{lemma}
		For a subgraph family $\F$ for directed graphs, and a filtering function $f$, it holds that {\em $\langle \F,f \rangle$-measure} is a centrality measure over directed graphs. 
	\end{lemma}
	
	We say that a centrality measure $\Ce$ is a {\em subgraph motif centrality measure} if there are a subgraph family $\F$ and a filtering function $f$ such that $\Ce$ is the $\langle \F,f \rangle$-measure, i.e., $\Ce = \subc{\F,f}$.


%Given a subgraph family for directed graphs $\F$ and a filtering function $f$, a subgraph motif centrality measure for directed graphs is the function $\Ce\langle\F,f\rangle$ such that $\Ce\langle\F,f\rangle(v,G)  = f(|\F(v,G)|)$ for every pair $(v,G)\in\vg$. We say that an arbitrary centrality measure for digraphs $\Ce$ is a subgraph motif centrality for digraphs if there exists a subgraphs family $\F$ and a filtering function $f$ such that for every $(v,G)$, $\Ce(v,G) = \subc{\F,f}(v,G)$.

We can define the sets $\val{G}{n}(\Ce)$ and $\val{}{n}(\Ce)$ in exactly the same way as for undirected graphs. The key difference is that now we might have more values for a fixed integer $n$. In other words, in general, there are more pairs $(v,G)$ such that $|\A(v,G)|\leq n$ when $G$ is a directed graph rather than being undirected. Analogously, we can define the notion of $\Ce$-colorability for a measure $\Ce$ over directed graphs. 
%
We are now ready to state our main characterizations for directed graphs, which are similar to the ones for undirected graphs.

\begin{theorem}\label{the:characterization-directed}
	Consider a centrality measure $\Ce$ for digraphs. The following are equivalent:
	
	\begin{enumerate}
		\item $\Ce$ is a subgraph motif centrality measure for digraphs.
		
		\item For every $n>0$, $|\val{}{n}(\Ce)|\leq n+1$.
	\end{enumerate}
\end{theorem}


\begin{theorem}
	Consider a centrality measure $\Ce$ for digraphs. The following are equivalent:
	
	\begin{enumerate}
		\item $\Ce$ is a subgraph motif centrality measure for digraphs relative to the induced ranking.
		
		\item Every finite set $S \subseteq \vg$ is $\Ce$-colorable.
		
		\item $\vg$ is $\Ce$-colorable
	\end{enumerate}
\end{theorem}


The above statements look the same as Theorems~\ref{the:characterization} and~\ref{the:characterization-ranking}. Note, however, that they are semantically different since all the underlying notion (such as $\val{}{n}(\Ce)$ and $\vg$ are for directed graphs).
%
Interestingly, the proofs are identical with those for Theorems~\ref{the:characterization} and~\ref{the:characterization-ranking}.
%
We can finally state a result, analogous to Proposition~\ref{pro:coloring-to-non-uniform-bvp}, for directed graphs, which essentially states that the non-uniform bounded value property for directed graphs is a necessary condition for a measure for digraphs being subgraph motif relative to induced ranking.



\begin{proposition}\label{pro:coloring-to-non-uniform-bvp-directed}
	Consider a centrality measure $\Ce$ for digraphs. If there is a precoloring of $\vg$ that is non-uniformly $\Ce$-injective, then $\Ce$ enjoys the non-uniform bounded value property.
\end{proposition}

\subsection*{Monotonic Subgraph Motif Measures for Digraphs}

%In the same way we did for undirected graphs, we have characterization results for directed graphs when we restrict filtering functions to just monotonic ones.


We now state our main characterizations concerning monotonic subgraph motif measures for the case of directed graphs, which are similar to the ones for undirected graphs. Note that the sets $\bval{G}{n}(\Ce)$ and $\bval{}{n}(\Ce)$ are defined in the same way as for undirected graphs.


\begin{theorem}\label{the:monotonic-characterization-directed}
	Consider a centrality measure $\Ce$ for digraphs. The following are equivalent:
	
	\begin{enumerate}
		\item $\Ce$ is a monotonic subgraph motif centrality measure for digraphs.
		
		\item
		 For every $n>0$, $|\val{}{n}(\Ce)|\leq n+1 -|\bval{}{n}(\Ce)|$.
	\end{enumerate}
\end{theorem}

\begin{theorem}\label{the:characterization-monotonic-ranking-directed}
	Consider a centrality measure $\Ce$ for digraphs. The following are equivalent:
	
	\begin{enumerate}
		\item $\Ce$ is a monotonic subgraph motif centrality measure for digraphs relative to the induced ranking.
		
		\item For every digraph $G$ and $n>0$, $|\val{G}{n}(\Ce)|\leq n+1 -|\bval{G}{n}(\Ce)|$.
	\end{enumerate}
\end{theorem}


As for the non-monotonic case, the proofs of the above results are identical with those for Theorems~\ref{the:monotonic-characterization} and~\ref{the:monotonic-characterization-ranking}, respectively.
%
This is because the proofs only exploit the sizes of the sets $\val{G}{n}(\Ce)$, $\val{}{n}(\Ce)$, $\bval{G}{n}(\Ce)$ and $\bval{}{n}(\Ce)$ rather than the structure of their members.


We can finally show a result, analogous to Theorem~\ref{the:ranking-connected-graphs}, for directed graphs, which essentially provides a unifying framework for all centrality measures over digraphs as long as we focus on connected graphs, and we are only interested in the induced ranking.
%
The notation $\conC$ for a centrality measures $\Ce$ for digraphs is defined as for undirected graphs.


%\textbf{Note:} Proofs for the above characterizations over directed graphs are equivalent to the analogous ones in the case of undirected graphs. This can be seen from the fact that such proofs just depend on the sizes of sets $\val{n}{}(\Ce)$ and $\A(v,G)$ rather than the structure of the particular graphs involved.

\begin{theorem}\label{the:ranking-connected-graphs-monotonic-directed}
	For a centrality measure $\Ce$ for digraphs it holds that $\conC$ is a monotonic subgraph motif measure for digraphs relative to the induced ranking.
\end{theorem}

\begin{proof}
	The proof is along the lines of the proof for Theorem~\ref{the:ranking-connected-graphs}. 
	%we can build a similar subgraph motif measure for digraphs. 
	Given a connected digraph $G$, we build the equivalence relation $\equiv_G$ over $V(G)$ in the same way as in the proof of Theorem~\ref{the:ranking-connected-graphs}. 
	%
	Due to the fact that $G$ is a connected digraph, for every $v \in V(G)$, $|\A(v,G)| \geq |V(G)|$ since between $v$ and any other node $u\in V(G)$ there exists a connected subgraph containing $v$ and $u$. Such a subgraph can be seen as an undirected path in the multi-graph $\text{UN}(G)$. We can now define a subgraph family $\F$ such that, for every $(v,G)$ with $[v]_{\equiv_{G}} = C_i$, $|\F(v,G)| = i-1$, ensuring that $\F$ is closed under isomorphism by exploiting the same idea as in the proof of Theorem~\ref{the:characterization}.
	%
	Finally, with the filtering function $f$ such that $f(i) = i+1$, it is easy to verify that $\rank(\Ce) = \rank(\subc{\F,f})$.
\end{proof}

\subsection*{Classification}

We proceed to perform a classification as the one performed in Section~\ref{sec:classification} for undirected graphs. It turned out that the classification for digraphs is identical to the one for undirected graphs (see Tables~\ref{tab:classification} and~\ref{tab:classification-monotonic}) apart from one case already discussed at the end of Section~\ref{sec:classification}, that is, the negative result $\times[\mathit{trees}]$ for $\eigenvector$ in both Tables~\ref{tab:classification} and~\ref{tab:classification-monotonic}. Although we can show that for directed graphs, $\eigenvector$ is not a (monotonic) subgraph motif centrality measure, it remains open whether these negative results hold even for directed trees.
%
Despite the fact that the classification for digraphs is the same as the one for undirected graphs, the underlying proofs are different since now we need to work with directed graphs, and the versions of the centrality measures in question that operate in digraphs.

%and the definitions of the centrality mesaures for directed definitions for each centrality measure.


%\subsection*{Stress}

\medskip

\noindent \paragraph{Stress.} We define the set of shortest paths from a node $v$ to a node $u$ in a digraph $G$ as $S_{G}(v,u)=\{\pi_{vu}\subseteq G\mid |\pi_{vu}| = d_{G}(v,u)\}$.
%
For a node $w \in V(G)$, the set of shortest paths from $u$ to $v$ going through $w$ is the set $S_{G}^{w}(v,u) = \{\pi_{vu}\in S_{G}(v,u)\mid w\in\pi_{vu}\}$. The {\em stress centrality} of a vertex $v \in V(G)$ is
\[
\mathsf{Stress}(v,G)\ =\ \displaystyle\sum_{(u,w)\in (V(G)/\{v\})^2}|S_{G}^{v}(u,w)|.
\]


\begin{proposition}\label{pro:directed-stress}
	$\stress$ is a monotonic subgraph motif measure for directed graphs.
\end{proposition}

\begin{proof}
In the same way as we did for undirected graph, we define the family of shortest paths going through $v$ in $G$ as \[
\mathsf{S}(v,G)\ =\ \bigcup_{u,w \in V(G) \setminus \{v\}} \left\{G_\pi \mid \pi \in S_{G}^{v}(u,w)\right\},
\]
$G_\pi$ is the subgraph induced by the path $\pi$ in $G$. We also consider the filtering function $id$, i.e., the identity function over $\mathbb{N}$, which is monotonic. Clearly, for every $(v,G) \in \vg$,
\[
\stress(v,G)\ = \subc{\mathsf{S}, f}(v,G),
\]
and the claim follows.
 %Nevertheless, the filtering function in the directed case is $f(x)= x$ because directed paths differentiate a starting and ending point. Finally, it is easy to see that $\stress(v,G) = \subc{\mathsf{S}, f}(v,G)$ for every pair $(v,G)$.
\end{proof}



%\subsection*{All subgraphs}
\noindent \paragraph{All-Subgraphs.} The all-subgraphs centrality measure can be defined for digraphs in the obvious way. It is easy to see that:


\begin{proposition}
	$\allsub$ is a monotonic subgraph motif measure for directed graphs.
\end{proposition}

\begin{proof}
	The $\allsub$ measure for digraphs simply counts weakly connected subgraphs, and the filtering function is $\log_2$. Therefore, $\allsub(v,G) = \log_2(|\A(v,G)|)$, for every pair $(v,G)$, and the claim follows.
\end{proof}


%\subsection*{Degree}
\medskip

\noindent \paragraph{Degree.} Given a digraph $G$ and a vertex $v \in V(G)$, the {\em degree centrality} of $v$ in $G$ is
\[
\mathsf{Degree}(v,G)\ =\ |\text{OUT}(v,G)| + |\text{IN}(v,G)|.
\]
We can show the following result:


\begin{comment}
\textbf{In-Degree centrality.} For a directed graph $G$ and a node $v$ in $V(G)$, we degine the in-degree centrality of $v$ in $G$ as $$\mathsf{In-degree}(v,G) = |\text{IN}(v,G)|.$$


\textbf{Out-Degree centrality.} For a directed graph $G$ and a node $v$ in $V(G)$, we degine the in-degree centrality of $v$ in $G$ as $$\mathsf{Out-degree}(v,G) = |\text{OUT}(v,G)|.$$

\textbf{Degree centrality.} For a directed graph $G$ and a node $v$ in $V(G)$, we degine the degree centrality of $v$ in $G$ as $$\mathsf{Degree}(v,G) = |\text{OUT}(v,G)| + |\text{IN}(v,G)|.$$
\end{comment}


\begin{proposition}
	$\degree$ is a monotonic subgraph motif measure for directed graphs.
\end{proposition}


\begin{proof}
	Consider the subgraph family $\mathsf{D}$ such that, for every $(v,G) \in \vg$,
	\[
	\mathsf{D}(v,G)\ =\ \{(\{v,u\},\{(v,u)\})\mid u\in\text{OUT}(v,G)\}\cup\{(\{v,u\},\{(u,v)\})\mid u\in\text{IN}(v,G)\} 
	\]
	and the filtering function $id$ that is the identity over $\mathbf{N}$, i.e., $id(x)= x$, which is monotonic. It is clear that $\mathsf{Degree}(v,G) = id(|\mathsf{D}(v,G)|)$, and the claim follows.
	%just counts the amount of children and parents of $v$ which is equivalent to $\degree$.
\end{proof}


%\subsection*{Cross-Clique connectivity}

%\medskip

\noindent \paragraph{Cross-Clique.}
The cross-clique centrality measure~\cite{everett1998analyzing} was introduced in the context of analyzing virus and information propagation. It is defined as the amount of cliques containing a certain vertex. 
%
Given a digraph $G$ and a vertex $v \in V(G)$, we define the set $\mi{Cl}(v,G) = \{S\in \A(v,G)\mid S \text{ is a clique}\}$. The {\em cross-clique centrality} of $v$ in $G$ is
\[
\clique(v,G)\ =\ |\mi{Cl}(v,G)|.
\]
It is straightforward to see that the following holds:

\begin{proposition}
	$\clique$ is a subgraph motif measure for directed graphs.
\end{proposition}


\begin{proof}
	We consider the subgraph family $\mathsf{K}(v,G) = \{S\in \A(v,G)\mid S\text{ is a clique}\}$ and the identity filtering function $id$. Clearly, $\clique(v,G) = id(|\mathsf{K}(v,G)|)$, for every pair $(v,G)$, and the claim follows.
\end{proof}


%\subsection*{Closeness}

\noindent \paragraph{Closeness.} For a digraph $G$ and vertices $u,v \in V(G)$, the distance from $u$ to $v$ in $G$ is $d_G(u,v)=  \displaystyle\min\{|\pi_{uv}|\mid \pi_{uv}\text{ is a path from }u\text{ to v}\}$. Then, we define the sum of distances for v in $G$ as $\text{SD}(v,G) = \displaystyle\sum_{u\in K_v(G)/\{v\}}d_{G}(v,u)$. Finally, we define closeness centrality as
\[
\mathsf{Closeness}(v,G)\ =\ \displaystyle\frac{1}{\text{SD}(v, G)}.
\]
By definition, the $\closeness$ centrality for a pair $(v,G)$ such that $|K_{v}(G)| = 1$ is $0$.


\begin{proposition}
 $\closeness$ is not a subgraph motif measure (relative to the induced ranking) for directed graphs. \end{proposition}

\begin{proof}
	As we did for Proposition~\ref{pro:closeness}, we will show that $\closeness$ does not satisfy the bounded value property nor the non-uniform bounded value property. 
	%
	For the former, we consider a set $S \subsetneq \vg$ such that, with $A_n =\{\closeness(v,G)\mid (v,G)\in S \text{ and } |\A(v,G)|\leq n\} $, it holds that $|A_n| > n+1$. This is enough to prove that $|\val{}{n}(\closeness)|> n+1$ since $A_n\subseteq \val{}{n}$.
	%
	Consider the set $\Sigma_{n} = \{\text{SD}(v,G)\mid (v,G)\in S \text{ and } |\A(v,G)|\leq n\}$. Observe that $|\val{}{n}(\closeness)|\leq n+1$ iff $|\Sigma_{n}|\leq n+1$ because $\closeness(v,G)=\displaystyle\frac{1}{\text{SD}(v,G)}$ for every $(v,G)\in \vg$. Therefore, it suffices to show that $|\Sigma_n| > n+1$. The rest of the proof proceed in two main steps:
	
	\begin{enumerate}
		\item For every $j>0$, it is easy to see that for the extreme of the line graph $\text{SD}(1, L_j) = \displaystyle\frac{j\cdot j-1}{2}$ while $|\A(1, L_j)| = j$. Therefore, it is clear that for $i,j\in [n]$ such that $i\not= j$, $\text{SD}(1,L_i)\not=\text{SD}(1,L_j)$. Therefore, $|\Sigma_n| > n$ if we add the isolated vertex and the pairs $\{(1, L_j)\mid j\in\{1,...,n\}\}$ to our set $S$.
		
		\item It remains to show that there exists $n>0$ for which $|\Sigma_n| > n+1$. Therefore, we just need to find one pair $(v',G')$ such that $|\A(v',G')|\leq n$ and $\sd(v',G')\not\in \{\sd(1,L_i)\mid i\in\{1,...,n\}\}$. This is the case for $n=5$. Observe that for the center of the star graph with $3$ nodes $(1,S_3)$ we have that $|\A(1 ,S_3)| = 4$, whereas $\sd(2,S_3) = 2$. Consider now the digraph $H=\{\{1,2,3,4\},\{(1,2),(2,3),(2,4)\}\}$. For the leaf node $1$ in $H$ we have $|\A(1,H)|=5$, whereas $\sd(1,H)=5$. At the same time, there is no $i\in\{1,...,5\}$ such that $\sd(1,L_i) \in\{2,5\}$. This means for $S= \{(1,L_1),(1,L_2),(1, L_3),(1,L_4),(2,S_3),(1,H)\}$, $|\val{}{4}(\closeness)| = |\Sigma_4| \geq |\{\sd(v,G)\mid (v,G)\in S\}| > 5$.
	\end{enumerate}

To show that $\closeness$ does not satisfy the non-uniform bounded value property we exploit the fact that it is local and closed under isomorphism.
% 
Gather all the pairs of $S$ inside one disconnected graph, where each connected component is isomorphic to one of the graphs used for the previous proof. In such a graph, $|\val{G}{5}| = 6$, which leads to a contradiction due to Proposition~\ref{pro:coloring-to-non-uniform-bvp-directed}.
\end{proof}


%\subsection*{Harmonic}

\noindent \paragraph{Harmonic.} The {\em harmonic centrality} for directed graphs is defined as follows:
\[
\harmonic(v,G)\ =\ \begin{cases}
0 & \text{ if }|K_{v}(G)| = 1\\
&\\
\displaystyle\sum_{u \in V(G) \setminus \{v\}}\frac{1}{d_{G}(v,u)} & \text{otherwise}.
\end{cases}
\]
Notice that whenever $u\not\in K_{v}(G)$, $d_{G}(v,u) = \infty$, and thus, we assume that $\frac{1}{d_{G}(v,u)} = 0$.

\begin{proposition}
	The following hold:
	
	\begin{enumerate}
		\item $\harmonic$ is not a subgraph motif measure for directed graphs. 
		
		\item $\harmonic$ is not a subgraph motif measure relative to the induced ranking for directed graphs.
	\end{enumerate}
	
\end{proposition}

\begin{proof}
	\underline{Item (1).} We follow the same strategy as in the proof of Proposition~\ref{pro:harmonic}.
	%
	We first observe that $\harmonic(1,L_i) = \sum_{j=1}^{i-1}\displaystyle\frac{1}{j}$. Therefore, for $i \geq 1$, we have that $\harmonic(1,L_{i+1}) = \harmonic(1,L_i) + \displaystyle\frac{1}{i}$. This means $\harmonic(1,L_i)\not=\harmonic(1,L_j)$ for every $i,j$ with $i \neq j$. Hence, $|\val{}{n}(\harmonic)| \geq n-1$. Since $\harmonic(1,L_1) = 0$, we get that $|\val{}{n}(\harmonic)| \geq n$. 
	%
	Now, let $n = 6$. Consider the following pairs: $(2, H_1)$ and $(2, H_2)$ where $H_1 = \{\{1,2,3\},\{(2,1),(2,3)\}\}$ and $H_2 = \{\{1,2,3,4\},\{(2,1),(2,3),(3,4)\}\}$. We first observe that, for $n > 0$,
	\[
	\harmonic(2, H_1)\ =\ 2\ >\ \sum_{i=1}^{n-1}\displaystyle\frac{1}{i}\ =\ \harmonic(1, L_n).
	\]
	Moreover, we have that
	\[
	\harmonic(2, H_2)\ =\ 1 + 1 + \frac{1}{2}\ =\ 2.5. 
	\]
	Therefore, $|\val{}{6}(\harmonic)| \geq 7$, which means $\harmonic$ violates the bounded value property for $n = 6$. Thus, by Theorem~\ref{the:characterization-directed}, we conclude that $\harmonic$ is not a subgraph motif measure for directed graphs. This hold even for trees since every graph used above is a tree.
	
	\medskip
	
	\underline{Item (2).} By Proposition~\ref{pro:coloring-to-non-uniform-bvp-directed}, it suffices to show that $\harmonic$ does not enjoy the non-uniform bounded value property.
	%
	To this end, we follow the same idea as in the proof of Proposition~\ref{pro:closeness-ranking}. Roughly speaking, we gather all the graphs employed above to prove that $|\val{}{6}(\harmonic)|\geq 7$ in one disconnected graph $G$. Then, by exploiting the fact that $\harmonic$ is closed under isomorphism and local (see Definition~\ref{def:locality}), we can show that $|\val{G}{6}(\harmonic)| \geq 7$.
\end{proof}



%\subsection*{PageRank}

\noindent \paragraph{PageRank.}  Given a graph $G$ with $V(G)= \{v_1,\ldots,v_{|V(G)|}\}$, we define the adjacency matrix of $G$ as the matrix $A_{G}$ such that ${A_{G}}_{ij}=1$ if $(v_i,v_j)\in E(G)$. 
%
We then define $\textbf{P}$ as the column-stochastic matrix such that:
\[
\textbf{P}_{ij}\ =\ \displaystyle\frac{{A_{G}}_{ij}}{|N_G(i)|}.
\]
In other words, $\textbf{P}$ contains the probabilities of jumping from node $i$ to node $j$ during a random walk over $G$. Let $\mathbf{v}$ be a stochastic vector $(\mathbf{1}^T\mathbf{v} = 1)$, and let $0 < \alpha < 1$ be a teleportation parameter. Then, the {\em ($\mathbf{v},\alpha$)-PageRank vector} is defined as the vector $x_{\mathbf{v},\alpha}$ that solves the equation $(I-\alpha \textbf{P})x = (1-\alpha)\mathbf{v}$. 
%
Now, given a graph $G$ with $V(G)= \{v_1,\ldots,v_{|V(G)|}\}$, the {\em PageRank centrality} of $v_i$ in $G$ is defined as
$$
\pagerank(v_i,G) = x_{0.8,\mathbf{u}}[i],
$$
where $\mathbf{u} = \mathbf{1} \cdot \frac{1}{|V(G)|}$.
%
Several variations of $\pagerank$ have been proposed in the literature. In particular, if we do not force $x_{0.8,\mathbf{u}}$ to be a probability distribution, we can ask that the sum of centrality values inside a connected component is equal to the number of nodes in that component. Therefore, this give rise to the local version of $\pagerank$, denoted $\mathsf{LPR}$. We call it local since the values in a connected component are the same regardless of the graph.

\begin{proposition}
	The following hold:
	
	\begin{enumerate}
		\item $\pagerank$ is not a subgraph motif measure for directed graphs. 
		
		\item $\pagerank$ is not a subgraph motif measure relative to induced ranking for directed graphs. 
	\end{enumerate} 
	
\end{proposition}
\begin{proof}
	It suffices to consider the local version of $\pagerank$ since $\rank(\pagerank) = \rank({\mathsf{LPR}})$.
	
	\medskip
	
	\underline{Item (1).}
	It can verified that $\val{L_1}{5}(\mathsf{LPR}) = \{1\}$, $\val{L_2}{5}(\mathsf{LPR}) = \{1, 1.80\}$, $\val{L_3}{5}(\mathsf{LPR}) = \{1, 1.80, 2.44\}$, $\val{L_4}{5}(\mathsf{LPR}) = \{1, 1.80, 2.44, 2.95\}$, $\val{L_5}{5}(\mathsf{LPR}) = \{1, 1.80, 2.44, 2.95, 3.36\} $ and $\val{S_3}{5}(\mathsf{LPR})=\{1, 2.60\}$.
	%
	Moreover, for the digraph $H = (\{1,2,3,4\}, \{(2 ,1),(2, 3),(2,4)\})$, we have that  $\val{H}{5}(\mathsf{LPR}) = \{1.0, 1.27\}$
	% 
	Therefore,
	\[
	\{1, 1.80, 2.44, 2.95, 3.36, 2.60, 1.27\}\ \subseteq\ \val{}{5}(\mathsf{LPR}).
	\]
	Thus, $|\val{}{5}(\mathsf{LPR})| \geq 7$, which implies that $\mathsf{LPR}$ does not enjoy the bounded value property. Hence, by Theorem~\ref{the:characterization-directed}, we conclude that $\mathsf{LPR}$ is not a subgraph motif measure. This holds even if we focus on trees since every graph considered is a tree.
	
	
	\medskip
	
	\underline{Item (2).} By Proposition~\ref{pro:coloring-to-non-uniform-bvp-directed}, it suffices to show that $\mathsf{LPR}$ does not enjoy the non-uniform bounded value property.
	%
	To this end, we follow the same idea as in the proof of Proposition~\ref{pro:closeness-ranking}. Roughly speaking, we gather all the graphs employed above to prove that $|\val{}{5}(\mathsf{LPR})|>7$ in one disconnected graph $G$. Then, by exploiting the fact that $\mathsf{LPR}$ is closed under isomorphism and local (see Definition~\ref{def:locality-directed}), we can show that $|\val{G}{5}(\mathsf{LPR})| \geq 7$, and the claim follows.
\end{proof}



%\subsection*{EigenVector}

\noindent \paragraph{EigenVector.} Given a graph $G$ with $V(G)= \{u_1,...,u_{|V(G)|}\}$, we define the adjacency matrix of $G$ as the matrix $A_{G}$ such that ${A_{G}}_{ij}=1$ if $(u_i,u_j)\in E(G)$. 
Let $\lambda_{\max}(G)$ be the greatest eigenvalue of $A_G$.
%
We define the unique $L^2$ normalized eigenvector associated with $\lambda_{\max}(G)$ as $\mathbf{v}_{\max}$.
%
The {\em eigenvector centrality}~\cite{bonacich1987power} of $u_i$ in $G$ is the $i$-th entrance of $\mathbf{v}_{\max}$:
\[
\eigenvector(u_i,G)\ = \mathbf{v}_{\max}^{i}.
\]

\begin{proposition}\label{pro:eigenvector-directed}
	$\eigenvector$ is not a subgraph motif measure for directed graphs.
\end{proposition}

\begin{proof}
	We first prove the following: given a disconnected graph $G$ with $n = |\comp(G)|$, for each component $S$ of the set $M = \{S \in \comp(G)\mid \lambda_{\max}(G[V(S)]) = \lambda_{\max}(G)\}$, we have that
	$
	|\{\eigenvector(v,G)\mid v \in S\}| =  |\val{G[V(S)]}{}(\eigenvector)|.
	$ 
	%
	In other words, each component with the same maximum eigenvalue as $G$ will have the same amount of values as the component seen as a connected graph. On the other hand, we know that $\eigenvector$ must be a unitary vector. Therefore, if $G$ has multiple connected components with the maximum eigenvalue $\lambda_{\max}$, in order to give values to every vertex in those components, the vector is forced to give different values than those given to the component seen as a connected graph. 
	
	Given a graph $G$, we can order its vertices $V(G) = \{v_1,\ldots,v_n\}$ in such way that, if $\comp(G) = \{S_1,\ldots,S_k\}$, then, for every $m \in \{1,\ldots,k\}$, there exists $I_m=\{i_m, i_m +1, i_m+2,\ldots,i_m +|S_m|-1\}\subseteq \{1,\ldots,n\}$ such that $\{v_{s}\}_{s\in I_m} = S_m$. 
	%
	Therefore, the rows and columns of the adjacency matrix of $G$, $A_G$, are ordered such that there are square sections in the diagonal in $A_G$ where the $i$-th square section is the adjacency matrix of $G[V(S_i)]$, $A_{G[V(S_i)]}$. Out of these square sections the matrix $A_{G}$ just have values $0$ since vertices in different components have no connections between them. 
	%
	Now, for each $S_m \in M$, we know that if $b_m^{\max}$ is the eigenvector associated with $\lambda_{\max}$ in $G[V(S_m)]$, then the vector $v_{m}^{\star} = (0,0,\ldots,b_m^{\max}(1),\ldots,b_m^{\max}(|S_{m}|),0,\ldots,0)$ is a an eigenvector with eigenvalue $\lambda_{\max}$ for $A_G$ such that $v_m^{\star}(i_m+j)=b_m^{\max}(j-1)$ for $j\in\{0,\ldots,|S_m|-1\}$. This implies that any linear combination of the vectors $v_m^{\star}$ will by an eigenvector for $A_G$ with eigenvalue $\lambda_{\max}$. Finally, we have that the unique vector $v^{\star} = c_1v_{1}^{\star} + c_2v_{2}+\ldots+v_{|M|}^{\star}$ such that $\|v^{\star}\|=1$ is the eigenvector for $\eigenvector$ centrality in $G$. In other words, for each node $v_i\in V(G)$, then $\eigenvector(v,G) = v^{\star}(i)$. As we showed, the vector $v^{\star}$ assign values for every connected component $S_m\in M$ which are proportional to $b_m^{\max}$. Therefore, we can conclude that for every $n$, $|\val{G}{n}(\eigenvector)| \geq  |\bigcup_{S\in M}\val{G[V(S)]}{n}(\eigenvector)|$.
	%
	Now, we will construct a sequence of graphs $G_i$ in order to prove that $|\val{}{4}(\eigenvector)| > 5$. For $i >1 $, define the digraph $G_i = (\{0,1,\ldots,i\}, \{(i,i+1),(i+1,i)\mid i\mod2 = 0\})$. For $i\geq2$, we have that $G_i$ contains $\lceil i/2 \rceil$ connected components. Each one is isomorphic to cycle with two nodes $C_2$ whenever $i\mod 2 = 0$. Since the cycle with two nodes has maximum eigenvalue $\lambda_{\max} = 1$ the eigenvector $v^{\star} = (1/\sqrt{i},1/\sqrt{i},\ldots,1/\sqrt{i})$ is the eigenvector centrality vector for $G_i$. This fact implies that $|\val{}{4}(\eigenvector)| \geq |\bigcup_{j=1}^{i}\val{G_i}{n}(\eigenvector)| = i $ for every $i>0$. In other words, the set $\val{}{4}(\eigenvector)$ has infinitely many values which contradicts the bounded value property.
	%
	Thus, by Theorem~\ref{the:characterization-directed}, we conclude that $\eigenvector$ is not a subgraph motif measure for directed graphs.
\end{proof}

By Theorem~\ref{the:ranking-connected-graphs-monotonic-directed}, $\eigenvector$ is a subgraph motif measure relative to the induced ranking over connected graphs. We proceed to strengthen this result by showing that it holds over a broader class of graphs than the class of connected graphs. Let
\begin{multline*}
\mathbf{K}_1\ =\ \{G \in \mathbf{G} \mid \text{for every } G_1,G_2 \in \comp(G),\\ \lambda_{\max}(G[V(G_1)]) =\lambda_{\max}(G[V(G_2)])=\lambda_{\max}(G) \text{ implies } G_1 \cong G_2\}.
\end{multline*}
It is easy to verify that every connected graph belongs to $\mathbf{K}_1$, and that $\mathbf{K}_1$ may contain disconnected graphs. We show that:


\begin{proposition}\label{pro:eigenvector-ranking-directed}
	$\eigenvector$ is a subgraph motif measure relative to the induced ranking when restricted to $\mathbf{K_1}$.
\end{proposition}


\begin{proof}
	From the proof of Proposition~\ref{pro:eigenvector-directed}, we know that for every component of $M(G) = \{S\in \comp(G)\mid \lambda_{\max}(G[V(S)]) = \lambda_{\max}(G)\}$, the eigenvector centrality assigns the same amount of values to the connected component as it seen as a connected graph. On the other hand, if $S\not\in M(G)$, then, for every vertex $v \in V(S)$, we have that $\eigenvector(v,G) = 0$. Note that, whenever two graphs are isomorphic they have the same values in every eigenvector. Values are just permuted depending on the isomorphism you map each graph to the other. Therefore, we have that, for every graph $G \in \mathbf{K}_1$, there exists $S \in M(G)$ such that $\val{G}{n}(\eigenvector) = \val{G[V(S)]}{n}(\eigenvector)$. In other words, when $\eigenvector$ is restricted to $\mathbf{K}_1$ it behaves like $\con\eigenvector$. Hence, we can use the same subgraph family and filtering function employed in the proof of Theorem~\ref{the:ranking-connected-graphs-monotonic-directed} with the addition of value $0$ for vertices outside $S$ in $M(G)$.
\end{proof}



%\subsection*{Betweenness}

\noindent
\paragraph{Betweenness.} Betweenness centrality for $v$ in $G$ is defined as \[
\mathsf{Betweenness}(v,G)\ =\ \displaystyle\sum_{(u,w)\in (V(G)/\{v\})^2}\displaystyle\frac{|S_{G}^{v}(u,w)|}{|S_{G}(u,w)|}.
\]
If for some pair $(u,w)$ the set $|S_G(u,w)| = 0$, then $\displaystyle\frac{|S_{G}^{v}(u,w)|}{|S_{G}(u,w)|} =0$ by definition.

\begin{proposition}
	$\betweeness$ is a subgraph motif measure for directed graphs when restricted to trees.
\end{proposition}

\begin{proof}
	Proof is analogous to the one of Proposition~\ref{pro:betweenness-positive-trees}. For any tree $T$, and any pair of nodes $u\not=v$ in $V(T)$, $|S_T(u,v)|\leq 1$. Therefore, we can use the family of subgraphs defined in Proposition~\ref{pro:directed-stress} and the identity filtering function over $\mathbb{N}$ to prove that $\betweeness$ is a subgraph motif measure when restricted to trees.
\end{proof}

\begin{proposition}\label{pro:betweenness-directed}
	The following hold:
	
	\begin{enumerate}
		\item $\betweeness$ is not a monotonic subgraph motif measure for directed graphs, even if we focus on connected graphs.
		\item $\betweeness$ is not a monotonic subgraph motif measure relative to the induced ranking for directed graphs.
	\end{enumerate}
\end{proposition}

\begin{proof}
	\underline{Item (1).} We are going to show that $\betweeness$ does not enjoy the monotonic bounded value property, and thus, by Theorem~\ref{the:monotonic-characterization-directed}, it is not a monotonic subgraph motif measure.
	%
	For $n\geq1$, consider the connected graph $H_n = (V_n, E_n)$, where
	\begin{eqnarray*}
	V_n &=& \{1,2,...,n+2\}\\
	E_n &=& \{(1, i) \mid i \in\{3,4,\ldots,n+2\}\}\cup\{(2, i)\mid i \in\{3,4,.\ldots,n+2\}\}. 
	\end{eqnarray*}
	It can be verified that $\betweeness(3, H_n) = \frac{2}{n}$. However, for $n>1$, $|\A(3, H_n)| > 4$. Therefore, we have that
	\[
	|\val{}{4}(\betweeness)| + |\bval{}{4}(\betweeness)|\ >\ 5,
	\]
	which implies that $\betweeness$ does not enjoy the monotonic bounded value property.
	
	\medskip
	
	\underline{Item(2).} By Theorem~\ref{the:characterization-monotonic-ranking-directed}, it suffices to show that $\betweeness$ does not enjoy the non-uniform bounded value property.
	%
	Since $\betweeness$ is closed under isomorphism and local, we will use the same strategy as we did in analogous proofs. In particular, we define the graph $G$ as the minimal graph with the following property: for every graph $G' \in \{H_1,H_2,\ldots,H_5, H_6\}$, there exists a component $G''\in\comp(G)$ such that $G''$ is isomorphic to $G'$. We can then show that
	\[
	|\val{G}{4}(\betweeness)| + |\bval{G}{4}(\betweeness)|\ >\ 5,
	\]
	which implies that $\betweeness$ does not enjoy the non-uniform monotonic bounded value property, and the claim follows.
\end{proof}


==> app-preliminaries.tex <==
In this preliminary section, we present some auxiliary notions that have not been introduced in the main body of the paper, but are needed for the proofs given in the appendix. In particular, we are going to introduce some special classes of graphs (lines and stars), and the property of locality.
%a couple of useful properties of centrality measures (closure under isomorphism and locality).



\subsection*{Special Graphs}
%

The {\em line graph} with $m>0$ vertices, denoted $L_m$, is the undirected graph $(V,E)$, where 
\[
V\ =\ \{1,\ldots,m\} \quad \text{and} \quad E = \bigcup_{i \in \{1,\ldots,m-1\}}\{\{i,i+1\}\}.
\]


\noindent The {\em star graph} with $m>0$ vertices, denoted $S_m$, is the undirected graph $(V,E)$, where
\[
V\ =\ \{1,\ldots,m\} \quad \text{and} \quad E\ =\ \bigcup_{i \in \{2,\ldots,m\}} \{\{1,i\}\}.
\]
We refer to the vertex $1$ as the center of $S_m$.

\begin{comment}
\subsection*{Closure Under Isomorphism}
%

We say that two graphs $G_1$ and $G_2$ are {\em isomorphic}, denoted $G_1\simeq G_2$, if there exists a bijective function $h: V(G_1) \to V(G_2)$ such that $\{v,u\} \in E(G_1)$ iff $\{h(v),h(u)\}\in E(G_2)$.
%
Furthermore, given the vertices $v_1 \in V(G_1)$ and $v_2 \in V(G_2)$, we say that the pairs $(v_1, G_1)$ and $(v_2,G_2)$ are isomorphic, denoted $(v_1, G_1) \simeq (v_2,G_2)$, if $G_1\simeq G_2$ witnessed by $h$, and $h(v_1)= v_2$.
%
We are now ready to define the property of being closed under isomorphism for centrality measures.


\begin{definition}\label{def:closed-under-iso}
	Consider a centrality measure $\Ce$. We say that $\Ce$ is {\em closed under isomorphism} if, for every two pairs $(v_1,G_1) \in \vg$ and $(v_2,G_2) \in \vg$, $(v_1, G_1) \simeq (v_2,G_2)$ implies $\Ce(v_1,G_1) = \Ce(v_2,G_2)$. \hfill\markfull
\end{definition}


In simple words, the above property states that the values assigned by a measure to the vertices of a graph do not depend on the names of the vertices, but only on the structure of the graph; hence, the above property is sometimes called {\em anonymity}.
\end{comment}

\subsection*{Locality}
%

We recall the so-called locality property. Recall that, given a graph $G$ and a set of vertices $S \subseteq V(G)$, we write $G[S]$ for the subgraph of $G$ induced by $S$. Moreover, for a vertex $v \in V(G)$, we write $K_v(G)$ for the set of vertices occurring in the component of $G$ containing the vertex $v$.
%
The definition of locality follows:

\begin{definition}\label{def:locality}
	A centrality measure $\Ce$ is {\em local} if, for every pair $(v,G) \in \vg$, $\Ce(v,G) = \Ce(v,G[K_v(G)])$. \hfill\markfull
\end{definition}


In simple words, the above property tells us that the value assigned by a measure $\Ce$ to a vertex $v$ in a graph $G$ depends only on the component $G' \in \comp(G)$ that contains $v$, i.e., during the calcuation of $\Ce(v,G)$, $\Ce$ considers only the component $G'$.



==> app-sec3.tex <==
\subsection*{Proof of Proposition~\ref{pro:no-subc-measure-ranking}}

Let $\hat{G} = (\{v_1,v_2,v_3,v_4\},\{\{v_1,v_2\}\})$.
%
Consider the centrality measure $\Ce$ defined as follows:
\[
\Ce(v,G)\ =\ \begin{cases}
1 & G \neq \hat{G}\\
i+1 & G = \hat{G} \text{ and } v=v_i \text{ for } i \in [4].
\end{cases}
\]
It suffices to focus on the set of graphs $\gr^\star = \{G_v \mid v \in \ins{V}\} \cup \{\hat{G}\} \subseteq \gr$.
%
By providing an argument similar to that in the proof of Proposition~\ref{pro:no-subc-measure}, we can show that, for every subgraph family $\F$ and filtering function $f$, there exist $1 \leq i < j \leq 4$ such that $\subc{\F,f}(v_i,\hat{G}) = \subc{\F,f}(v_j,\hat{G})$. Therefore, $\{((v_i,\hat{G}),(v_j,\hat{G})),((v_j,\hat{G}),(v_i,\hat{G}))\} \subseteq \rank(\subc{\F,f})$.
%
On the other hand, only $((v_i,\hat{G}),(v_j,\hat{G}))$ belongs to $\rank(\Ce)$.
%
Consequently, for every subgraph family $\F$ and filtering function $f$, $\rank(\Ce) \neq \rank(\subc{\F,f})$, and the claim follows.



\begin{comment}
\subsection{Example for uniform not monotonic}

Define measure $C$ as follows where $H$ is the graph in figure~\ref{ex:nonUniform}:

$$C_1(v,G) = \begin{cases}
	1 & G\not= H\wedge v\in V(G)\\
	2 & (v,G) = (v_1, H)\\
	3 & (v,G) = (v_2, H)\\
	4 & (v,G) = (v_3, H)\\
	-\infty & \text{ otherwise.}
\end{cases}$$

For any node $v$, notice that $C_1(v,G_v) = 1$ since $G_v\not= H$. Now, we can see that $C$ is not a motif measure because there are not enough families to represent such values. Suppose for some family $\F$ and function $f$ we have $C_1=C_{\F,f}$. For the pair $(v,G_v)$ we must have $|\F(v,G_v)|\in\{0,1\}$ because $|\asg(v,G)| = 1$. On the other hand, for $|\F(v_1, H)|\not=|\F(v_2, H)| \in\{0,1,2\}$ since $|\asg(v_1,H)| = |\asg(v_2, H)| = 2$ and $C(v_1, H)\not= C(v_2, H)$. Finally, for $(v_3, H)$ it must be the case that $|\F(v_3, H)|\not=|\F(v, G_v)|$ since $C(v_3,H)\not= C(v,G_v)$. In conclusion, we have $4$ different values but $3$ possible sizes for the families. Therefore, $\F$ can not exist.

\begin{figure}[h]
	\Ceentering
	\input{../Figures/graph-ex1}
	\Ceaption{Graph $H$ and values for $C$.}
	\label{ex:nonUniform}
\end{figure}

If we analyse the ranking defined by $C$ this is a complete different story. We can choose the following family $$\F(v, G)=\begin{cases}
	\{\} & G\not= H\wedge v\in V(G)\\
	\{\} & (v,G)= (v_1, H)\\
	\{G_{v_2}, K_{v_2}(H)\} & (v, G) =(v_2, H)\\
	\{(\{v\},\emptyset)\} & (v,G) = (v_3, H)
\end{cases}$$

and define the function $f =\{(0,1), (1,3), (2, 2)\}$. The reader can corroborate that for every graph $G$, then $\preceq^{G}_{C_1} = \preceq^{G}_{C_{\F,f}}$.

\subsection{Example for ranking motif centrality}

Define measure $C$ as follows where $S$ is in figure~\ref{ex:nonmotif}:

$$C_2(v,G) = \begin{cases}
	1 & G\not= H\wedge v\in V(G)\\
	2 & (v,G) = (v_1, S)\\
	3 & (v,G) = (v_2, S)\\
	4 & (v,G) = (v_3, S)\\
	5 & (v,G) = (v_4, S)
\end{cases}$$

\begin{figure}[h]
	\Ceentering
	\input{../Figures/graph-ex2}
	\Ceaption{Graph $S$ and values for $C_2$.}
	\label{ex:nonmotif}
\end{figure}

We will show that $C_2$ is not a sub graph motif centrality, even when we compare rankings. By the same reason as in the previous example, $C_2$ can not be defined by any family $\F$ and function $f$. Now, if we look at the ranking $\preceq^{S}_{C_2}$, we got that for any $\F$ and $f$ then for some $v_i\not= v_j$ we will have that $C_{\F,f}(v_i, S) = C_{\F,f}(v_j, S) $ which means that $\preceq^{S}_{C_2}\not=\preceq^{S}_{C_{\F,f}}$.
\end{comment}

==> app-sec4.tex <==
\subsection*{Proof of Theorem~\ref{the:characterization}}
%

$\underline{(1 \Rightarrow 2).}$  By contradiction, assume that $\Ce$ does not enjoy the bounded value property, namely there exists an integer $n\geq1$ such that $|\val{}{n}(\Ce)| > n+1$. 
%
By hypothesis, $\Ce$ is a subgraph motif centrality measure, and thus, there exist a subgraph family $\F$ and a filtering function $f$ such that the following holds: for every $(v,G)\in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$. 
%
We now define the set 
\[
B_n\ =\ \left\{|\F(v,G)|\mid (v,G)\in \vg \text{ and } |\A(v,G)| \leq n\right\}. 
\]
Clearly, $|B_n| \leq n+1$ since $\F(v,G) \subseteq \A(v,G)$. 
%
We also define the function $h : \val{}{n}(\Ce) \to B_n$ such that
\[
h(\Ce(v,G))\ =\ |\F(v,G)|.
\]
By the pigeonhole principle, $h$ is not injective, i.e., there exist $\Ce(v_1,G_1)$ and $\Ce(v_2,G_2)$ such that $\Ce(v_1,G_1) \neq \Ce(v_2,G_2)$ but $|\F(v_1,G_1)| = |\F(v_2,G_2)|$. This contradicts the fact that $\Ce(v_1,G_1) = f(|\F(v_1,G_1)|) \neq f(|\F(v_2,G_2)|) = \Ce(v_2,G_2)$.
	
\medskip

$\underline{(2 \Rightarrow 1).}$ The goal is to show that there exist a subgraph family $\F$ and a filtering function $f$ such that, for every $(v,G) \in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$.
%
We start by defining a total order $\preceq_{\Ce}$ over the set of values $\val{}{}(\Ce) = \bigcup_{i=1}^{\infty}\val{}{i}(\Ce)$. 
%
By definition, for every $n,m > 0$ such that $n \leq m$, it holds that $\val{}{n}(\Ce)\subseteq \val{}{m}(\Ce)$. In other words, as we increase the integer $n$ we are adding new values to the set $\val{}{n}(\Ce)$.
%
We can now define the binary relation $\preceq_{\Ce}$ over $\val{}{}(\Ce)$ as follows: for each $a,b \in \val{}{}(\Ce)$, if there exists $n$ such that $a \in \val{}{n}(\Ce)$ but $b \not\in \val{}{n}(\Ce)$ then $a \preceq_{\Ce} b$, if not, then $a \preceq_{\Ce} b$ if $a\leq b$. 
%
It is easy to see that $\preceq_{\Ce}$ is a total order over $\val{}{}(\Ce)$, and thus, it is a total order over $\val{}{n}(\Ce)$ for each $ n> 0$. For notational convenience, in the rest of the proof we assume that  $\val{}{}(\Ce) = \{a_1,a_2,a_3,\ldots\}$ and $a_1 \preceq_{\Ce} a_2 \preceq_{\Ce} a_3 \preceq_{\Ce} \cdots$.


By exploiting the total order $\preceq_{\Ce}$ over $\val{}{}(\Ce)$, we now define a subgraph family $\F$. Consider an arbitrary pair $(v,G) \in \vg$, and let $n = |\A(v,G)|$. 
%
By hypothesis, $\Ce$ enjoys the bounded value property, which in turn implies that $|\val{}{n}(\Ce)| \leq n+1$. Therefore, $\Ce(v,G) \in \left\{a_1,a_2,...,a_{|\val{}{n}(\Ce)|}\right\} = \val{}{n}(\Ce)$. %Here we ordered the set $\val{}{n}(\Ce)$ by the relation $\preceq_{\Ce}$. 
%
We further observe that $\A(v,G)$ is a finite set; let $\A(v,G) = \{S_1,S_2,\ldots,S_n\}$. 
%
Here we assume an arbitrary order for $\A(v,G)$ that has the following property: for every pair of nodes $(v',G')$ with $(v,G)\simeq (v',G')$, assuming that $\A(v',G') = \{S'_1,S'_2,\ldots,S'_n\}$, it holds that $(v,S_i)\simeq (v'_i,S'_i)$ for every $i\in\{1,\ldots,n\}$.
%
The subgraph family $\F$ is defined as follows:
\[
\Ce(v,G) = a_i \quad \text{implies} \quad \F(v,G) = \{S_1,...,S_{i-1}\}.
\]
This is indeed a subgraph family since $\F(v,G) \subseteq \A(v,G)$, while the chosen order for $\A(v,G)$ and the fact that $\Ce$ is (by definition) closed under isomorphism ensures closure under isomorphism. Notice that $|\F(v,G)| = i-1$ for $i \in \{1,\ldots,|\val{}{n}(\Ce)|+1\}$.
%
Finally, we define the filtering function $f : \mathbb{N} \to \val{}{}(\Ce)$ as follows: for each $i \in \mathbb{N}$,
\[
f(i)\ =\ a_{i+1}. 
\]
We proceed to show the following technical lemma, which essentially states that $\F$ and $f$ capture our intention:

\begin{lemma}\label{lem:correctness}
	For every $(v,G) \in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$.
\end{lemma}

\begin{proof}
	Let $n = |\A(v,G)|$. If $\Ce(v,G) = a_i\in \val{}{n}(\Ce)$, then $|\F(v,G)| = i-1$. Therefore, $f(|\F(v,G)|) = \subc{\F,f}(v,G) = \Ce(v,G)$.
	%
	Conversely, if $\subc{\F,f}(v,G) = a_i$, then $|\F(v,G)| = i-1$, and thus, by construction, $\Ce(v,G) = a_i$.
\end{proof}

By Lemma~\ref{lem:correctness}, we get that $\Ce$ is a subgraph motif measure, and Theorem~\ref{the:characterization} follows.


\begin{comment}
To prove that $2\implies 1$, in first place we need to give an order for the sets $\val{}{n}(\Ce)$. By definition we know that for any pair $n,m\in \mathbb{N}$ such that $n\leq m$ then $\val{}{n}(\Ce)\subseteq \val{}{m}(\Ce)$. Which means that as we increase $n$ we are adding new values to $\val{}{n}(\Ce)$. Define the set $\val{}{}(\Ce) = \bigcup_{i=1}^{\infty}\val{}{i}(\Ce)$. Then, we can order $\val{}{}(\Ce)$ with the following relation. For any $a,b \in \val{}{}(\Ce)$, $a\preceq_{\Ce} b$ if exists $n$ such that $a\in \val{}{n}(\Ce)$ but $b\not\in \val{}{n}(\Ce)$. Otherwise, $a\preceq_{\Ce} b$ if $a \leq b$. The relation $\preceq_{\Ce}$ is a total order for $\val{}{}(\Ce)$ which means that it is a total order in $\val{}{n}(\Ce)$ for all $ n>0$. From now on we will assume that $\val{}{}(\Ce) = \{a_1,a_2,...\}$ is ordered by $\preceq_C$.
	
\smallskip
Now, we want to define a family of substructures $\F$. Take an arbitrary pair $(v,G)$ such that $v\in V(G)$ and set $n =|\A(v,G)|$. By the structural axiom we know that $|\val{}{n}(C)|\leq n+1$. Therefore, $\Ce(v,G)\in\{a_1,a_2,...,a_{|\val{}{n}(\Ce)|}\}=\val{}{n}(\Ce)$. Here we ordered the set $\val{}{n}(\Ce)$ by the relation $\preceq_{\Ce}$. On the other hand, since $\A(v,G)$ is a finite set, we can set an arbitrary order as $\A(v,G) = \{S_1,S_2,...,S_n\}$. Now we can define the family as $\F(v,G) = \{S_1,...,S_{i-1}\}$ if $\Ce(v,G) = a_i$. This is a well defined family since $\F(v,G)\subseteq \A(v,G)$. Notice that $|\F(v,G)| = i-1$ for $i\in\{1,...,|\val{}{n}(\Ce)|+1\}$. 
	
\smallskip
Finally, we will define a function $f:\mathbb{N}\to \val{}{}(\Ce)$ as $f(i) = a_{i+1}$. From this point we just have to prove that $\Ce(v,G) = \subc{\F,f}(v,G)$ for every node $v$ and every graph $G$. If $\Ce(v,G) = a_i\in \val{}{n}(\Ce)$ for $n = |\A(v,G)|$, then $|\F(v,G)| = i-1$ which implies that $f(|\F(v,G)|)=\Ce(v,G)$. In the other direction, if $\subc{\F,f}(v,G) = a_i$ we know that $|\F(v,G)| = i-1$. Which by construction means that  $\Ce(v,G) = a_i$.
\end{comment}


\subsection*{Proof of Proposition~\ref{pro:closeness}}
%

Our goal is to show that $\closeness$ does not enjoy the bounded value property, and thus, by Theorem~\ref{the:characterization}, it is not a subgraph motif measure, as needed. To this end, we need to show that there is $n>0$ such that $|\val{}{n}(\closeness)| > n+1$.
%
For notational convenience, given a pair $(v,G) \in \vg$, let $\sd(v,G) = \sum_{u\in K_v(G)} d_G(v,u)$. We observe that, for each $n>0$, 
\[
|\val{}{n}(\closeness)|> n+1 \quad \text{iff} \quad |\underbrace{\{\textsc{SD}(v,G) \mid v \in V(G) \text{ and } |\A(v,G)| \leq n\}}_{\Sigma_n}| > n+1. 
\]
Therefore, it suffices to show that there is $n>0$ such that $|\Sigma_n| > n+1$.
%
The rest of the proof proceeds in two main steps:
% in what follows, we denote by $L_m$ the {\em line} of $m>0$ vertices, where $V(L_m) = \{1,\ldots,m\}$ and $E(L_m) = \{\{i,i+1\} \mid i \in [m-1]\}$:

\begin{enumerate}
\item For every $n>0$, it is easy to see that $\textsc{SD}(1,L_n) = \frac{n \cdot (n-1)}{2}$ and $|\A(1,L_n)| = n$. Therefore, it is clear that, for every $i,j \in [n]$ with $i \neq j$, $\textsc{SD}(1,L_i) \neq \sd(1,L_j)$, $|\A(1,L_i)| \leq n$, and $|\A(1, L_j)| \leq n$. Therefore, $|\Sigma_n| \geq n$.


\item It remains to show that there exists $n>0$ for which there are two pairs $(v_1,G_1),(v_2,G_2)$ of $\vg$ such that $|\A(v_1, G_1)|\leq n$ and $|\A(v_2, G_2)|\leq n$, but $\textsc{SD}(v_1,G_1) \neq \textsc{SD}(v_2, G_2) \neq \textsc{SD}(1,L_i)$, for every $i \leq n$, which implies that $|\Sigma_n| > n+1$, as needed. We proceed to show the latter for $n = 5$.
%
%Let $S_3$ be the star graph with $3$ leaves, where $V(S_3) = \{1,2,3,4\}$ and $E(S_3) = \{\{1,2\},\{1,3\},\{1,4\}\}$. 
It is easy to verify that the center of the star graph $S_4$
participates in eight connected subgraphs. Thus, any leaf vertex participates in $1 + 2^2 = 5$ connected subgraphs. 
%
Therefore, $|\A(i, S_4)| \leq 5$ for $i \in \{2,3,4\}$. On the other hand, if we look at the center vertex of $L_3$, that is, vertex $2$ of $L_3$, it participates in four connected subgraphs, and thus, $|\A(2, L_3)| \leq 5$.
%
Finally, we have that $\sd(1, S_4) = 5$, whereas $\sd(2, L_3) = 2$. Observe that there is no $i \in \{1,\ldots,5\}$ such that $\sd(1, L_i) \in \{2,5\}$, and thus, $|\Sigma_5| > 6$.
\end{enumerate}


\begin{comment}
In first place, for a pair $(v,G)$ define the value $\sd(v,G) = \sum_{u\in K_v(G)} d_G(v,u)$. This proof goes directly by proving that $\Celoseness$ does not satisfy the bounded value property. It is important to notice that for any $n>0$, $|\val{}{n}(\Celoseness)|> n+1$ if and only if $|\{\textsc{SD}(v,G) \mid (v,G)\in X_n\}|>n+1$ . Therefore, it is enough to prove that the sum of distances for pairs $(v,G)$ such that $|\A(v,G)|\leq n$ is not upper bounded by $n+1$. Now, for a fixed $n\geq 1$, define the sequence of line graphs as $\{L_i\}_{i=1}^{n}$ such that $V(L_i) = \{1,...,i\}$ and $1$ as the extreme node of $L_i$. We have that $\textsc{SD}(1,L_i) = i(i-1)/2$ while $|\A(1,L_i)| = i$. This means that for every $i\not= j \in \{1,...,n\}, \textsc{SD}(1,L_i)\not= \sd(1,L_j)$ but $|\A(1,L_i)| \leq n$ and $|\A(1, L_j)|\leq n$. This means that $|\val{}{n}(\Celoseness)|>n$. Therefore, we just need two more pairs $(v_1,G_1)$ and $(v_2,G_2)$ such that $|\A(v_1, G_1)|\leq n$ and $|\A(v_2, G_2)|\leq n$ but $\textsc{SD}(v_1,G_1) \not= \textsc{SD}(v_2, G_2)\not= \textsc{SD}(1,L_i)$ for every $i \leq n$. Set $n = 5$. Define the star graph with $3$ leaves $S_3$. The center of $S_3$ has $8$ subgraphs. Thus, any leaf will have $1 + 2^2 = 5$ connected subgraphs. Therefore, if $v$ is a leaf in $S_3$, then $|\A(v, S_3)|\leq 5$. On the other hand, if we look at the center of the line graph with $3$ nodes $L_3$, it has $4$ connected subgraphs surrounding it. Therefore, $|\A(2, L_3)|\leq 5$. Finally, we have that $\sd(v, S_3) = 5$ while $\sd(1, L_3) = 2$. For such values, there is no $i\in\{1,..,5\}$ such that $\sd(1, L_i) \in \{3,5\}$. Concluding that $|\val{}{5}(\textsc{Closeness})| > 6$ which contradicts the bounded value property.
\end{comment}

==> app-sec5.tex <==

\subsection*{Proof of Theorem~\ref{the:characterization-ranking}}


$\underline{(1 \Rightarrow 2).}$
Since, by hypothesis, $\Ce$ is a subgraph motif measure relative to the induced ranking, there are a subgraph family $\F$ and a filtering function $f$ such that $\rank(\Ce) = \rank(\subc{\F,f})$. Given a finite set $S \subsetneq \vg$, we define the function $\pc_S : S \rightarrow \mathbb{N}$ as follows: for every $(v,G) \in S$, $\pc_S(v,G) = |\F(v,G)|$. It is clear that $\pc_S$ is a precoloring of $S$ since, by definition, $\F(v,G) \subseteq \A(v,G)$, and thus, $\pc_S(v,G) \in \{0,\ldots,|\A(v,G)|\}$. It remains to show that $\pc_S$ is (i) non-uniformly $\Ce$-injective, and (ii) $\Ce$-consistent, which in turn implies that $S$ is $\Ce$-colorable:
\begin{itemize}
\item[(i)] Since $\rank(\Ce) = \rank(\Ce\langle\F,f\rangle)$, for every $(u_1, G),(u_2,G) \in S$, it holds that $\Ce(u_1, G) \neq \Ce(u_2,G)$ iff $\subc{\F,f}(u_1, G)\not=\subc{\F,f}(u_2, G)$. Therefore, $\pc_S(u_1,G) = |\F(u_1,G)| \neq |\F(u_2,G)| = \pc_S(u_2,G)$, which implies that $\pc_S$ is non-uniformly $\Ce$-injective.

\item[(ii)] By contradiction, assume that there exist $(v_1,G_1),(v_2,G_1),(u_1,G_2)$ and $(u_2,G_2)$ such that $\Ce(v_1,G_1)<\Ce(v_2,G_1)$ and $\Ce(u_1,G_2) >\Ce(u_2,G_2)$ but $\pc_S(u_1,G_2) = \pc_S(v_1,G_1)$ and $\pc_S(v_2,G_1) = \pc_S(u_2,G_2)$. Therefore, $|\F(v_1,G_1)| = |\F(u_1,G_2)|$ and $|\F(v_2,G_1)| = |\F(u_2,G_2)|$. Consequently, using the fact that $\rank(\Ce) = \rank(\Ce\langle\F,f\rangle)$, $\subc{\F,f}(v_1,G_1) < \subc{\F,f}(v_2,G_1) = \subc{\F,f}(u_2,G_2)<\subc{\F,f}(u_1,G_2)=\subc{\F,f}(v_1,G_1)$, which is clearly a contradiction. Hence, $\pc_S$ is also $\Ce$-consistent.
\end{itemize}


%Fix a finite set $S\subset \mathbf{VG}$. We know there exists a family of subgraphs $\F$ and a filter function $f$ such that $\rank(\Ce) = \rank(C\langle\F,f\rangle)$. Define the function $g(v,G)= |\F(v,G)|$. We will prove that $g$ is a $\Ce-$ colouring for $S$. In first place, we know for every pair $(v,G)\in S$ then $g(v,G) = |\F(v,G)|\leq |\A(v,G)|$ since $\F(v,G) \subseteq \A(v,G)$. In other words, $g$ is a precoloring for $S$. In second place, since $\rank(\Ce) = \rank(C\langle\F,f\rangle)$, for $(u_1, G)$ and $(u_2,G)$ in $S$, we have that $C(u_1, G)\not=C(u_2,G)$ if and only if $\subc{\F,f}(u_1, G)\not=\subc{\F,f}(u_2, G)$. Therefore, $g(u_1,G) = |\F(u_1,G)|\not=|\F(u_2,G)| = g(u_2,G)$ implying $g$ is non-uniformly $\Ce-$injective. Finally, by contradiction suppose there exists $(v_1,G_1),(v_2,G_1),(u_1,G_2)$ and $(u_2,G_2)$ such that $\Ce(v_1,G_1)<\Ce(v_2,G_1)$ and $\Ce(u_1,G_2) >\Ce(u_2,G_2)$ but $g(u_1,G_2) = g(v_1,G_1)$ and $g(v_2,G_1)=g(u_2,G_2)$. Therefore, $|\F(v_1,G_1)| = |\F(u_1,G_2)|$ and $|\F(v_2,G_1)| = |\F(u_2,G_2)|$. In consequence, using the fact that $\rank(\Ce) = \rank(\Ce\langle\F,f\rangle)$, $\subc{\F,f}(v_1,G_1) < \subc{\F,f}(v_2,G_1) = \subc{\F,f}(u_2,G_2)<\subc{\F,f}(u_1,G_2)=\subc{\F,f}(v_1,G_1)$ which is clearly a contradiction. Therefore, $g$ is also $\Ce-$consistent.

\medskip

$\underline{(2 \Rightarrow 3).}$
The proof of this implication heavily relies on  Rado's Selection Principle (see Theorem~\ref{the:rados}).
%
By hypothesis, for each $S \in \mathcal{P}_{\mathsf{fin}}(\vg)$, there exists a precoloring of $S$, i.e., a function $\pc_S : S \rightarrow \mathbb{N}$, that is non-uniformly $\Ce$-injective and $\Ce$-consistent. Since, for every $(v,G) \in \vg$, $\A(v,G)$ is finite, we can conclude that the following holds: for every $(v,G) \in \vg$, the set $\{\pc_S(v,G) \mid S \in \mathcal{P}_{\mathsf{fin}}(\vg) \text{ and } (v,G) \in S\}$ is finite. This allows us to apply Theorem~\ref{the:rados} with $A = \vg$ and $B = \mathbb{N}$. Therefore, there exists a function $f : \vg \rightarrow \mathbb{N}$ such that, for every $S \in \mathcal{P}_{\mathsf{fin}}(\vg)$, there exists $S' \in \mathcal{P}_{\mathsf{fin}}(\vg)$ with $S \subsetneq S'$ and $f_{|S} = {\pc_{S'}}_{|S}$. 
%
By exploiting the latter property of the function $f$ guaranteed by Theorem~\ref{the:rados}, and the fact that, for each $S \in \mathcal{P}_{\mathsf{fin}}(\vg)$, $\pc_S$ is a precoloring of $S$ that is non-uniformly $\Ce$-injective and $\Ce$-consistent, we can show that (i) $f$ is a precoloring of $\vg$ that is (ii) non-uniformly $\Ce$-injective, and (iii) $\Ce$-consistent, which in turn implies item (3):
\begin{itemize}
	\item[(i)] For every pair $(v, G)\in\vg$, we have that $f(v,G) = \pc_S(v,G)$ for some set $S \in \mathcal{P}_{\mathsf{fin}}(\vg)$ such that $\{(v,G)\} \subsetneq S$. Since $\pc_S$ is a precoloring of $S$, we get that $f(v,G) = \pc_S(v,G) \in \{0,\ldots,|\A(v,G)|\}$, and thus, $f$ is a precoloring of $\vg$. 
	
	\item[(ii)] For every two pairs $(v_1,G)$ and $(v_2,G)$ such that $\Ce(v_1,G) \neq \Ce(v_2,G)$ we know there exists a finite set $S$ such that $\{(v_1,G),(v_2,G)\}\subsetneq S$ with $\pc_S(v_i,G) = f(v_i,G)$ for $i\in\{1,2\}$. Therefore, since $\Ce(v_1,G) \neq \Ce(v_2,G)$ and $\pc_S$ is non-uniformly $\Ce$-injective, we get that $f(v_1,G) = \pc_S(v_1,G) \neq \pc_S(v_2,G) = f(v_2,G)$. This implies that $f$ is non-uniformly $\Ce$-injective. 
	
	\item[(ii)] Finally, by contradiction, assume there are four pairs $(v_1,G_1),(v_2,G_1),(u_1,G_2)$ and $(u_2,G_2)$ in $\vg$ such that $\Ce(v_1,G_1)<\Ce(v_2,G_1)$ and $\Ce(u_2,G_2)<\Ce(u_1,G_2)$, but $f(v_1,G_1)=f(u_1,G_2)$ and $f(v_2,G_1)=f(u_2,G_2)$. We know that there exists a finite set $S'$ such that $S=\{(v_1,G_1),(v_2,G_1),(u_1,G_2),(u_2,G_2)\}\subsetneq S'$ with $f(v,G) = \pc_{S'}(v,G)$ for every $(v,G)\in S$. This implies that $\pc_{S'}$ is not $\Ce$-consistent, which is clearly a contradiction.
\end{itemize}
This completes the proof of the second implication.


%This goes by using theorem~\ref{the:rados}. Define $A = \vg$ and $B=\mathbb{N}$. By hypothesis we have a colouring $f_S$ for every finite set $S\subseteq \vg$. Since $A(v,G)$ is finite for every pair, we have that for every $(v,G)\in \vg$, the set $\{f_S(v,G)\mid S\in \mathcal{P}_{\mathsf{fin}}(\vg)\wedge (v,G)\in S\}$ is also finite. Therefore, there exists a colouring function $f:\vg\to\mathbb{N}$ such that for every finite set $S\subset\vg$, there exists a finite set $S'$ where $S\subset S'$ and for every $(v,G)\in S$ then $f(v,G) = f_{S'}(v,G)$. Now we just need to prove that $f$ is a colouring for $\vg$. In first place, take any pair $(v, G)\in\vg$, we have that $f(v,G) = f_{S}(v,G)$ for some finite $S$ such that $\{(v,G)\}\subset S$. Since $f_S(v,G)$ is a colouring for $S$, then $f(v,G) = f_S(v,G) \leq |\A(v,G)|$. Therefore, $f$ is as precoloring for $\vg$. In second place, for every two pairs $(v_1,G)$ and $(v_2,G)$ such that $C(v_1,G)\not=C(v_2,G)$ we know there exists a finite set $S$ such that $\{(v_1,G),(v_2,G)\}\subset S$ and $f_{S}(v_i,G) = f(v_i,G)$ for $i\in\{1,2\}$. Therefore, since $\Ce(v_1,G)\not=\Ce(v_2,G)$ and $f_S$ is a proper colouring, we know $f(v_1,G)=f_S(v_1,G)\not=f_S(v_2,G) = f(v_2,G)$. Which implies that $f$ is non-uniformly $\Ce-$injective. Finally, to prove the $\Ce-$consistency of $f$, suppose there exists four pairs $(v_1,G_1),(v_2,G_1),(u_1,G_2)$ and $(u_2,G_2)$ in $\vg$ such that $\Ce(v_1,G_1)<\Ce(v_2,G_1)$ and $\Ce(u_2,G_2)<\Ce(u_1,G_2)$ but $f(v_1,G_1)=f(u_1,G_2)$ and $f(v_2,G_1)=f(u_2,G_2)$. We know by the same argument there exists a finite set $S'$ such that $S=\{(v_1,G_1),(v_2,G_1),(u_1,G_2),(u_2,G_2)\}\subset S'$ such that $f(v,G) = f_{S'}(v,G)$ for every $(v,G)\in S$. Therefore, $f_{S}$ is not a proper coloring of $S'$ and we find a contradiction.


\medskip

$\underline{(3 \Rightarrow 1).}$ The goal is to devise a subgraph family $\F$ and a filtering function $f$ such that $\rank(\Ce) = \rank(\subc{\F,f})$, which in turn proves item $(1)$. By hypothesis, there exists a precoloring $\pc$ of $\vg$ that is non-uniformly $\Ce$-injective and $\Ce$-consistent. We define $\F$ in such way that, for every $(v,G) \in \vg$, $|\F(v,G)| = \pc(v,G)$; note that such a subgraph family exists since $\pc(v,G) \in \{0,\ldots,|\A(v,G)|\}$. Note that such a property can be satisfied by forcing $\F$ to be closed under isomorphism using the same idea as in the proof of Theorem~\ref{the:characterization}.
%
We now proceed to define the filtering function $f$. Let $R_{\pc}$ be the binary relation
\begin{multline*}
\{(i,j) \in \mathbb{N} \times \mathbb{N} \mid \text{ there are } (u,G), (v,G) \text{ in } \vg \text{ such that }\\ \Ce(u,G) < \Ce(v,G), \pc(u,G) = i, \text{ and } \pc(v,G) = j\}.
\end{multline*}
The fact that $\pc$ is non-uniformly $\Ce$-injective allows us to conclude that $R_\pc$ is irreflexive. Moreover, the $\Ce$-consistency of $\pc$ implies that $R_\pc$ is asymmetric.
%
Observe now that if we extend $R_\pc$ into a total order $R_{\pc}^{\star}$ over $\mathbb{N}$, and then show that $R_{\pc}^{\star}$ can be embedded into a carefully chosen countable subset $N$ of $\mathbb{R}$, then we obtain the desired filtering function $f$, which assigns real numbers to the sizes of the subgraph families assigned to the pairs of $\vg$ by $\F$ as dictated by the embedding of $R_{\pc}^{\star}$ into $N \subsetneq \mathbb{R}$.
%
We now explain how this is done.


The binary relation $R_\pc$ is first extended into the strict partial order $R_{\pc}^{+}$ by simply taking its transitive closure. Now, the fact that $R_{\pc}^{+}$ can be extended into a total order $R_{\pc}^{\star}$ over $\mathbb{N}$ follows by the {\em order-extension principle} (a.k.a.~{\em Szpilrajn Extension Theorem}), shown by Szpilrajn in 1930~\cite{szpi30}, which essentially states that every partial order can be extended into a total order.
%
It remains to show that $R_{\pc}^{\star}$ can be embedded into some countable set $N \subsetneq \mathbb{R}$. This is done via the {\em back-and-forth method}, a technique for showing isomorphism between countably infinite structures satisfying certain conditions.
%
We proceed by case analysis:

\begin{description}
	\item[Case 1.] Assume first that there exists a minimum and maximum element in the ordered set $(\mathbb{N},R_{\pc}^{\star})$, denoted $n_0$ and $n_1$, respectively. 
	%
	Consider a close range of the rational numbers $[a,b]\subseteq \mathbb{Q}$ with $a < b$. Fix any order of the set $\mathbb{N}-\{n_0,n_1\}=\{a_1,a_2,...\}$, and fix a different order of $[a,b]=\{b_1,b_2,...\}$. This is possible because both sets are countable. We proceed to define the order preserving embedding of $(\mathbb{N},R_{\pc}^{\star})$ to $([a,b],<)$. First, define $f(n_0) = a$ and $f(n_1) = b$. Now, the back and forth method goes as follow:
	\medskip
	\begin{enumerate}
		\item Take $a_i$ such that $i$ is the first index where $f(a_i)$ is not assign yet. Define $f(a_i)= b_j$ such that $b_j$ is the first element in the list without pre image from $f$, and respects the order embedding up to this point. In other words, for every $a_{k_1}$ and $a_{k_2}$ such that $f(a_{k_1})$ and $f(a_{k_2})$ are defined and $ a_{k_1}R_{\pc}^{\star} a_i R_{\pc}^{\star} a_{k_2}$, it holds that $f(a_{k_1})<b_j < f(a_{k_2})$.
		
		\item Repeat the previous step until we cover the whole set $\mathbb{N}$.
	\end{enumerate}
	\medskip
	Given $a_p$ and $a_q$ such that $a_pR_{\pc}^{\star}a_iR_{\pc}^{\star}a_q$ where $f(a_p)$ and $f(a_q)$ are both assigned, since $([a,b],<)$ is a dense order, for every two elements there is always another element in between. Therefore, we can always find $b_j$ as stated in the previous steps. In conclusion, we can map $(\mathbb{N},R_{\pc}^{\star})$ to $([a,b],<)$ respecting both orders, and $f$ is precisely the filtering function that we are looking for.
	
	\item[Cases 2, 3 and 4.]  In the remaining three cases, where $(\mathbb{N},R_{\pc}^{\star})$ has only a minimum element, only a maximum element, and no extreme elements, respectively, the same argument as above applies using the sets $\mathbb{Q}^{+}$, $\mathbb{Q}^{-}$ and $\mathbb{Q}$, respectively, instead of $[a,b]\subseteq \mathbb{Q}$ . 
\end{description}

It remains to show that $\rank(\subc{\F,f}) = \rank(\Ce)$ for the family $\F$ and filtering function $f$ defined above.
%
Take any two pairs $(v_1, G)$ and $(v_2,G)$ such that $\Ce(v_1, G)< \Ce(v_2, G)$. By definition, we have that $(\pc(v_1,G),\pc(v_2,G))\in R_{\pc}^{\star}$. This is equivalent to $f(\pc(v_1, G)) = f(|\F(v_1,G)|) < f(\pc(v_2,G))= f(|\F(v_2,G)|)$. Therefore, $\subc{\F,f}$ and $\Ce$ induce the same ranking inside each graph, and the claim follows.



%%%%%

\begin{comment}
We will need to define the a subgraph motif measure $\subc{\F,f}$ such that $\rank(\Ce) = \rank(\subc{\F,f})$. To this end, we will exploit the colouring $\pc:\vg\to \mathbb{N}$. In first place, select a subgraph family $\F$ such that for every $(v,G)$ then $|\F(v,G)|=\pc(v,G)$. Such a family must exist since $\pc(v,G) \leq |\A(v,G)|$ since $\pc$ is a proper colouring for $\vg$. In second place, we must find a filtering function $f$. Define the relation $R_{\pc}\subseteq \mathbb{N}^2$ such that $(i,j)\in R_{\pc}$ if there exists $(v_1,G)$ and $(v_2,G)$ in $\vg$ such that $\Ce(v_1,G) < \Ce(v_2,G)$ while $\pc(v_1,G)=i$ and $\pc(v_2,G) = j$. By $\Ce-$injectivity of $\pc$, we know relation $R_{\pc}$ is irreflexive and by Consistency it is easy to see that $R_{\pc}$ is asymmetric. Therefore, we will create a strict total order of $\mathbb{N}$ extending $R_{\pc}$ which will be later embedded into a subset of the real numbers. If such embed exists, it means we can map the sizes (or colours) of $\F$ into real numbers respecting the order inside each graph at the same time. I.e, the filtering function $f$ exists. We define the relation $R_{\pc}^{+}$ as the transitive closure of $R_{\pc}$. Therefore, $R_{\pc}^{+}$ is a partial order over $\mathbb{N}$ which has the same order as $R_{\pc}$ between colours that appear in the same graph. Finally, by the order extension principle, there exists an extension $R_{\pc}^\star$ of $R_{\pc}^{+}$ such that $R_{\pc}^{\star}$ is a total order of $\mathbb{N}$. Now, using the back and forth method we will prove that we can embed $R_{\pc}^{\star}$ into some set $S\subseteq\mathbb{R}$. In order to do this we will cover 4 different cases. Suppose in first case that there exists a minimum and maximum element in the set $(\mathbb{N},R_{\pc}^{\star})$ being $n_0$ and $n_1$ respectively. On the other hand, take any close range of the rational numbers $[a,b]\subseteq \mathbb{Q}$ such that $a < b$. Give any order to the set $\mathbb{N}-\{n_0,n_1\}=\{a_1,a_2,...\}$ and fix a different order of $[a,b]=\{b_1,b_2,...\}$. This is possible because both sets are countable sets. We will define the order preserving embedding of $(\mathbb{N},R_{\pc}^{\star})$ to $([a,b],<)$. First, define $f(n_0) = a$ and $f(n_1) = b$. Now, the back and forth method goes as follow:

\begin{enumerate}
	\item Take $a_i$ such that $i$ is the first index where $f(a_i)$ is not assign yet. Define $f(a_i)= b_j$ such that $b_j$ is the first element in the list without pre image from $f$ and respect the order embedding up to this point. This is, for every $a_{k_1}$ and $a_{k_2}$ such that $f(a_{k_1})$ and $f(a_{k_2})$ are defined and $ a_{k_1}R_{\pc}^{\star} a_i R_{\pc}^{\star} a_{k_2}$ then $f(a_{k_1})<b_j < f(a_{k_2})$.
	
	\item Repeat previous step until cover the whole set $\mathbb{N}$.
\end{enumerate}

Given $a_p$ and $a_q$ such that $a_pR_{\pc}^{\star}a_iR_{\pc}^{\star}a_q$ where $f(a_p)$ and $f(a_q)$ are both assigned, since $([a,b],<)$ is a dense order, for every two elements there is always another element in between. Therefore, we can always find $b_j$ as stated in the previous steps. In conclusion, we can map $(\mathbb{N},R_{\pc}^{\star})$ to $([a,b],<)$ respecting both orders and this $f$ we created is precisely the filtering function we need. In the other cases where $(\mathbb{N},R_{\pc}^{\star})$ has just a minimum element, just a maximum element or no extreme elements at all, the same argument can be done using the sets $\mathbb{Q}^{+}$, $\mathbb{Q}^{-}$ and $\mathbb{Q}$ respectively instead of $[a,b]$. Now, we just need to prove that $\rank(\subc{\F,f}) = \rank(\Ce)$ for the family $\F$ and filtering function $f$ we just defined. Take any two pairs $(v_1, G)$ and $(v_2,G)$ such that $\Ce(v_1, G)< \Ce(v_2, G)$. Therefore, by definition we know $(\pc(v_1,G),\pc(v_2,G))\in R_{\pc}^{\star}$. This is if and only if $f(\pc(v_1, G)) = f(|\F(v_1,G)|) < f(\pc(v_2,G))= f(|\F(v_2,G)|)$. Therefore, $\subc{\F,f}$ and $\Ce$ have the same ranking inside each graph.
\end{comment}
%\subsection*{Proof of Theorem~\ref{the:characterization-ranking} Item (1)}
%%
%
%
%
%We are going to devise a centrality measure that is not subgraph motif relative to the induced ranking, but it enjoys the non-uniform bounded value property.
%%
%Consider the graphs $G_1 = (\{v_1,v_2,v_3\},\{\{v_2,v_3\}\}), G_2 = (\{u_1,u_2,u_3\},\{\{u_2,u_3\}\})$ and $G_3 = (\{w_1,w_2,w_3\},\{\{w_2,w_3\}\})$. Observe that these three graphs have the same structure, that is, one isolated node and two nodes connected by an edge.
%%
%We now define the following centrality measure:
%\[
%\Ce(v,G) = \begin{cases}
%1 & (v,G) \in \{(v_1, G_1), (u_2,G_2), (w_3, G_3)\}\\
%2 & (v,G) \in \{(v_2, G_1), (u_3,G_2), (w_1, G_3)\}\\
%3 & (v,G) \in \{(v_3, G_1), (u_1,G_2), (w_2, G_3)\}\\
%1 & \text{otherwise.}
%\end{cases}
%\]
%Roughly speaking, $\Ce$ is defined in such a way that the position of the isolated vertex in the induced ranking is shifted. Indeed, in $\rank(C)$, $(v_1,G_1)$ comes first, $(w_1,G_3)$ comes second, and $(u_1,G_2)$ comes third.
%%
%It can be shown that $\Ce$ is not subgraph motif relative to the induced tanking since any subgraph motif measure will need too many values in $\val{}{n}(\Ce)$, for some $n\geq1$, in order to mimic $\rank(\Ce)$.
%%
%On the other hand, for every $i \in \{1,2,3\}$, we have that $|\val{G_i}{n}(\Ce)| \leq n+1$, and thus, $\Ce$ enjoys the non-uniform bounded value property, and the claim follows.
%
%
%\subsection*{Proof of Theorem~\ref{the:characterization-ranking} Item (2)}
%%
%
%Consider a centrality measure $\Ce$ that is subgraph motif relative to the induced ranking. By definition, there are a subgraph family $\F$ and a filtering function $f$ such that $\rank(\Ce) = \rank(\subc{\F,f})$.
%%
%Assume, by contradiction, that $\Ce$ does not enjoy the non-uniform bounded value property, that is, there exist a graph $G$ and an integer $n \geq 1$ such that $|\val{G}{n}(\Ce)| > n+1$. 
%%
%Since $\rank(\Ce) = \rank(\subc{\F,f})$, we have that, for every $(v_1, G),(v_2, G) \in \vg$, $\Ce(v_1, G)<\Ce(v_2, G)$ iff $\subc{\F,f}(v_1, G)<\subc{\F,f}(v_2, G)$. Therefore, we can conclude that $|\val{G}{n}(\subc{\F,f})| = |\val{G}{n}(\Ce)|$, and thus
%\[
%|\val{}{n}(\subc{\F,f})|\ \geq\ |\val{G}{n}(\subc{\F,f})|\ =\ |\val{G}{n}(\Ce)| > n+1.
%\]
%This means that $\subc{\F,f}$ does not enjoy the bounded value property. Hence, by Theorem~\ref{the:characterization}, we get that $\subc{\F,f}$ is not a subgraph motif measure, which leads to contradiction. Consequently, $\Ce$ enjoys the non-uniform bounded value property, as needed.


\begin{comment}
In first place, suppose that there exists a subgraph motif centrality $\subc{\F,f}$ such that $\rank(\Ce) = \rank(\subc{\F,f})$. By contradiction assume there is a graph $G$ and $n\geq 1$ such that $|\val{G}{n}(\Ce)| > n+1$. Since $\rank(\Ce) = \rank(\subc{\F,f})$ we have that for every $(v_1, G)$ and $(v_2, G)$, then $\Ce(v_1, G)<\Ce(v_2, G)$ if and only if $\subc{\F,f}(v_1, G)<\subc{\F,f}(v_2, G)$. Therefore, $|\val{}{n}(\subc{\F,f})|\geq |\val{G}{n}(\subc{\F,f})| = |\val{G}{n}(\Ce)| > n+1$ which means by theorem~\ref{the:characterization} that $\subc{\F,f}$ is not a subgraph motif measure.
\end{comment}


%	 To prove that 2) implies 1) we will construct a function $f$ and a family $\F$ such that $\rank(\Ce) =\rank(\subc{\F,f})$ where $\subc{\F,f}$ is a subgraph motif centrality. Fix an arbitrary graph $G$. Since $G$ is finite, there must exists $n_0\geq 1$ such that $\val{G}{n}(\Ce) = \val{G}{n_0}(\Ce)$ for every $n \geq n_0$. At the same time, we can order $\val{G}{n_0}(\Ce) = \{a_1,...,a_{|\val{G}{n_0}(\Ce)|}\}$ following the order $\preceq_{\Ce}$ defined in the same way as in the proof of theorem~\ref{the:characterization}. Therefore, for every $v\in V(G)$, $\A(v,G)=\{S_1,...,S_{|\A(v,G)|}\}$ we define $\F(v,G) = \{S_1,...,S_{i-1}\}$ if $\Ce(v,G) = a_i$. Finally, in order to define the filter function $f$ first we order the set $\val{}{}(\Ce) = \Ceup_{i=1}^{\infty}\val{G_i}{}(\Ce) = \{b_1,b_2,...\}$ such that $b_i<b_j$ if $i<j$. $f$ is defined such that $f(|\F(v,G)|) = j$ if $\Ce(v,G) = b_j$. 	 
%%	  For a fixed graph $G$, we define the equivalence relation $\equiv_G$ such that for every $v,u$ in $V(G)$ then $v \equiv_G u$ if and only if $\Ce(v,G) = \Ce(u, G)$. Now, we can order the set of equivalence classes as $V(G)\slash_{\equiv_{G}} =\{c_1,...,c_m\}$ such that for every $i<j$ where $c_i = [v]_{\equiv_G}$ and  $c_j = [u]_{\equiv_G}$ then $\Ce(v, G) < \Ce(u, G)$. Define the family $\F$ such that $|\F(v,G)| = i-1$ if $c_i = [v]_{\equiv_G}$. We define the filter function $f$ such that $f(i) = i+1$. 
%In order to prove that measure $\Ce^{\star}=\subc{\F, f}$ is well defined, suppose by contradiction there exists a graph $G$ and node $v\in V(G)$ such that $\Ce(v,G) = a_i$ but $|\A(v,G)| = n < i-1$. Because we ordered the set $\val{G}{n_0}(\Ce)$ using $\preceq_{\Ce}$, we know that for ever $j\leq i$, then $a_j\in \val{G}{n}$. Therefore, $|\val{G}{n}| \geq i > n+1$ which contradicts the non uniform property. Finally, we must prove that $C^{\star}$ is a subgraph motif centrality. Since $\mathcal{G}^{V}$ is a countable set, we can order it arbitrarily as $\mathcal{G}^{V} = \{G_1, G_2,...\}$. Notice that $\val{}{n}(C^{\star}) = \displaystyle\bigcup_{i = 1}^{\infty} \val{G_i}{n}(\Ce^{\star})$ for every $n\geq1$. Now, because of how we defined $\Ce^{\star}$, for every two graphs $G_i, G_{j}$ we have that 
%	 
%	 \begin{equation}\label{eq:localcardinality0}
%	 	|\val{G_i}{n}(\Ce^{\star}) \Ceup \val{G_j}{n}(\Ce^{\star})|=  \max\{|\val{G_i}{n}(C^{\star})|, |\val{G_j}{n}(\Ce^{\star})|\}.
%	 \end{equation} At the same time, the fact that $\Ce$ enjoys the non uniform property implies that $C^{\star}$ also satisfies it. Therefore, 
%	 \begin{equation}\label{eq:localcardinality1}
%	 	\max\{|\val{G_i}{n}(\Ce^{\star})|, |\val{G_j}{n}(\Ce^{\star})|\} \leq n+1.
%	 \end{equation}
%	 Equations~\ref{eq:localcardinality0} and \ref{eq:localcardinality1} imply by induction that for any $k\geq 1$ then $\left|\displaystyle\bigcup_{i = 1}^{k} \val{G_i}{n}(\Ce^{\star})\right| \leq n+1$. Therefore, we have that $|\val{}{n}(\Ce^{\star})|\leq n+1$ concluding that $\Ce^{\star}$ enjoys the bounded value property.
%	 
%	 \smallskip
%	 To finish this proof, we will prove that $\rank(\Ce) = \rank(\Ce^{\star})$. Fix a graph $G$ and nodes $u,v$ in $V(G)$. If $a_j = \Ce(u, G)\leq \Ce(v, G)=a_i$. Therefore, $\Ce^{\star}(u, G) = j \leq i = \Ce^{\star}(v, G)$. In the other direction, if $\Ce^{\star}(u, G) = i \leq j = \Ce^{\star}(v, G)$ then $\Ce_{\F, r}(u,G) \leq C_{\F,r}(v,G)$ by definition of $\Ce^{\star}$.

\subsection*{Proof of Proposition~\ref{pro:coloring-to-non-uniform-bvp}}

Let $pc$ be the non-uniform $\Ce$-injective precoloring of $\Ce$, which exists by hypothesis.
%
Consider a graph $G$, and an integer $n>0$. Define the set
\[
S_n\ =\ \{pc(v,G)\mid |\A(v,G)|\leq n\}. 
\]
In other words, $S_n$ collects all the colors assigned by $pc$ to vertices with at most $n$ connected subgraphs around them. We then have that $|\val{G}{n}(\Ce)|\leq |S_n|$ since $pc$ is non-uniformly $\Ce$-injective. 
%
Since $pc$ is a precoloring, $S_n \subseteq \{0,\ldots,n\}$, and thus, $|S_n|\leq n+1$, as needed.



\subsection*{Proof of Proposition~\ref{pro:non-uniform-bvp-not-sufficient}}
%

We are going to devise a centrality measure that is not subgraph motif relative to the induced ranking, but it enjoys the non-uniform bounded value property.
%
Consider the graphs
\begin{eqnarray*}
G_1 &=& (\{v_1,v_2,v_3,v_4,v_5,v_6\},\{\{v_2,v_3\},\{v_4,v_5\},\{v_5,v_6\}\})\\ 
G_2 &=& (\{v_1,v_2,v_3,v_4,v_5,v_6,v_7\},\{\{v_2,v_3\},\{v_4,v_5\},\{v_5,v_6\}\})\\ 
G_3 &=& (\{v_1,v_2,v_3,v_4,v_5,v_6,v_7,v_8\},\{\{v_2,v_3\},\{v_4,v_5\},\{v_5,v_6\}\}). 
\end{eqnarray*}
that are graphically represented as follows:

\begin{figure}[h]\label{figure:e4c2}
	\centering
	
	\begin{subfigure}[b]{0.3\textwidth}
		\begin{tikzpicture}[x=2cm,y=3cm] % change these values to adjust the size of a figure
		\tikzset{     
			e4c node/.style={circle,draw,minimum size=0.5cm,inner sep=0}, 
			e4c edge/.style={sloped,above,font=\footnotesize}
		}
		\node[e4c node] (1) at (0.00, 0.90) {$v_1$}; 
		\node[e4c node] (2) at (0.00, 1.20) {$v_2$}; 
		\node[e4c node] (3) at (0.50, 1.20) {$v_3$}; 
		\node[e4c node] (4) at (1.00, 1.50) {$v_4$}; 
		\node[e4c node] (5) at (0.50, 1.5) {$v_5$}; 
		\node[e4c node] (6) at (0.00, 1.5) {$v_6$}; 
		\node[] (graph) at (-0.5,1.2) {$G_1$};
		
		\path[draw,thick]
		(2) edge[e4c edge]  (3)
		(4) edge[e4c edge]  (5)
		(5) edge[e4c edge]  (6)
		;
		\end{tikzpicture}
		
		% \caption{Optional caption.} 
		% Created with Editor4Centralities.
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
	
	
	\begin{tikzpicture}[x=2cm,y=3cm] % change these values to adjust the size of a figure
	\tikzset{     
		e4c node/.style={circle,draw,minimum size=0.5cm,inner sep=0}, 
		e4c edge/.style={sloped,above,font=\footnotesize}
	}
	\node[e4c node] (1) at (0.5, 0.9) {$v_1$}; 
	\node[e4c node] (2) at (0.00, 1.20) {$v_2$}; 
	\node[e4c node] (3) at (0.50, 1.20) {$v_3$}; 
	\node[e4c node] (4) at (1.00, 1.50) {$v_4$}; 
	\node[e4c node] (5) at (0.50, 1.5) {$v_5$}; 
	\node[e4c node] (6) at (0.00, 1.5) {$v_6$}; 
	\node[e4c node] (7) at (0.00, 0.90) {$v_7$}; 
	\node[] (graph) at (-0.5,1.2) {$G_2$};
	
	\path[draw,thick]
	(2) edge[e4c edge]  (3)
	(4) edge[e4c edge]  (5)
	(5) edge[e4c edge]  (6)
	;
	\end{tikzpicture}
	
	% \caption{Optional caption.} 
	% Created with Editor4Centralities.
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
	\begin{tikzpicture}[x=2cm,y=3cm] % change these values to adjust the size of a figure
	\tikzset{     
		e4c node/.style={circle,draw,minimum size=0.5cm,inner sep=0}, 
		e4c edge/.style={sloped,above,font=\footnotesize}
	}
	\node[e4c node] (1) at (0.00, 1.05) {$v_1$}; 
	\node[e4c node] (2) at (0.00, 1.35) {$v_2$}; 
	\node[e4c node] (3) at (0.50, 1.35) {$v_3$}; 
	\node[e4c node] (4) at (1.00, 1.65) {$v_4$}; 
	\node[e4c node] (5) at (0.50, 1.65) {$v_5$}; 
	\node[e4c node] (6) at (0.00, 1.65) {$v_6$}; 
	\node[e4c node] (7) at (0.50, 1.05) {$v_7$}; 
	\node[e4c node] (8) at (1, 1.05) {$v_8$}; 
	\node[] (graph) at (-0.5,1.35) {$G_3$};
	
	\path[draw,thick]
	(2) edge[e4c edge]  (3)
	(4) edge[e4c edge]  (5)
	(5) edge[e4c edge]  (6)
	;
	\end{tikzpicture}
	
	% \caption{Optional caption.} 
	% Created with Editor4Centralities.
	\end{subfigure}
\end{figure}


\noindent Observe that these three graphs have the same structure modulo some additional isolated vertices. In particular, they consist of some isolated vertices, two vertices connected by an edge, and a line of three vertices.
%
We now define the following function:
\[
\Ce(v,G) = \begin{cases}
1 & (v,G) \in \{(v_1, G_1), (v_2,G_2), (v_2, G_3)\}\\
2 & (v,G) \in \{(v_2,G_1), (v_1,G_2), (v_4, G_3)\}\\
3 & (v,G) \in \{(v_3, G_1), (v_3,G_2), (v_5, G_3)\}\\
4 & (v,G) \in \{(v_5, G_1), (v_5,G_2), (v_1, G_3)\}\\
1 & \text{otherwise.}
\end{cases}
\]
Roughly speaking, $\Ce$ is defined in such a way that the position of the isolated vertex in the induced ranking is shifted. Indeed, in $\rank(\Ce)$, $(v_1,G_1)$ comes first, $(v_1,G_2)$ comes second, and $(v_1,G_3)$ comes fourth. As usual, in this proof we consider an extended version of $\Ce$ that is closed under isomorphism and is defined over every pair of $\vg$. 
%
We have manually verified that $\Ce$ is not subgraph motif relative to the induced ranking. In particular, every subgraph motif measure will need too many values in $\val{}{n}(\Ce)$, for some $n\geq1$, in order to mimic $\rank(\Ce)$. 
%In particular, the vertex $v_5$ will need an extra value in every possible family we could assign by assigning colours from pairs with less to more subgraphs surrounding them.
%
On the other hand, for every $i \in \{1,2,3,4\}$, $|\val{G_i}{n}(\Ce)| \leq n+1$, and thus, $\Ce$ enjoys the non-uniform bounded value property, and the claim follows.


\subsection*{Proof of Proposition~\ref{pro:closeness-ranking}}
%

We are going to show that there exists a graph $G$ such that $|\val{G}{5}(\closeness)| > 6$. This implies that $\closeness$ does not enjoy the non-uniform bounded value property, and thus, by item (2) of Theorem~\ref{the:characterization-ranking}, it is not a subgraph motif measure relative to the induced ranking, as needed.
%
Consider the graphs $L_1,L_2,\ldots,L_5, S_4$. 
%Recall from the proof of Proposition~\ref{pro:closeness} that $L_i$ is the line with $i$ vertices, while $S_3$ is the star graph with three leaves.
%
We define the graph $G$ as the minimal graph with the following structural property: for every graph $G' \in \{L_1,L_2,\ldots,L_5, S_4\}$, there exists a component $G'' \in \comp(G)$ that is isomorphic to $G'$.
%
By employing an argument similar to that in the proof of Proposition~\ref{pro:closeness}, and exploiting the fact that $\closeness$ is closed under isomorphism (see Definition~\ref{def:centrality-measure}) and local (see Definition~\ref{def:locality}), we can show that $|\val{G}{5}(\closeness)| > 6$.

%\andreas{Here we exploit the fact that $\Celoseness$ is closed under isomorphism. Is this correct? Do we use this property in other proofs for other centrality measures?}

\begin{comment}
Take every graph $G_i$ used in the proof of proposition~\ref{pro:closeness}. We can define the graph $G$ as the minimal graph such that for every $i$, there exists a connected component $S\in\Ceomp(G)$ such that $S\Ceong G_i$. The definition of $\Celoseness$ implies that $|\val{G}{5}(\Celoseness)| > 6$ which means $\Celoseness$ can not be a subgraph motif measure respect to induced ranking.
\end{comment}


\subsection*{Proof of Theorem~\ref{the:ranking-connected-graphs}}
%

We are going to define a subgraph family $\F$ and a filtering function $f$ such that $\rank(\Ce) \cap \vcg^2 = \rank(\subc{\F,f}) \cap \vcg^2$, which in turn implies that $\conC$ is a subgraph motif measure relative to the induced ranking, as needed.
%
Consider an arbitrary connected graph $G$. We first observe that, for every $v \in V(G)$, it holds that $|\A(v, G)|\geq |V(G)|$ since every path from $v$ to any other vertex in $G$ is a connected subgraph containing $v$. 
%
We then define the equivalence relation $\equiv_G$ over $V(G)$ as follows:  $v \equiv_G u$ if $\Ce(v,G) = \Ce(u,G)$. Let $V(G)/_{\equiv_G} = \{C_1,\ldots,C_m\}$ be the equivalence classes of $\equiv_G$. We can assume, without loss of generality, that, for every $i,j \in [m]$, with $C_i = [v]_{\equiv_G}$ and $C_j = [u]_{\equiv_G}$, $i<j$ implies $\Ce(v,G)< \Ce(u, G)$.
%
We then define the subgraph family $\F$ in such a way that, for every vertex $v \in V(G)$, $|\F(v,G)|= i-1$ if $[v]_{\equiv_G} = C_i$.\footnote{Note that for pairs $(u,G')$, where $G'$ is a non-connected graph, we can simply define $\F(u,G')$ as the empty set since it is irrelevant what $\F$ does over non-connected graphs.} Note that such a subgraph family $\F$ always exists since, as discussed above, $|\A(v,G)|\geq |V(G)|$, but we have that $|V(G)/_{\equiv_G}| \leq |V(G)|$. Note also that we can ensure that $\F$ is closed under isomorphism by using the same idea as in the proof of Theorem~\ref{the:characterization}.
%
Finally, we define the filtering function $f$ in such a way that, for every $i \in \{0,\ldots,m-1\}$, $f(i) = i+1$. 
%
It is now not difficult to verify that indeed $\rank(\Ce) \cap \vcg^2 = \rank(\subc{\F,f}) \cap \vcg^2$.


\begin{comment}
Take any connected graph $G$. Since $G$ is connected, for every $v$ in $V(G)$, $|\A(v, G)|\geq |V(G)|$ because every path from $v$ to any other node is a connected subgraph containing $v$. Now, we can define the equivalence relation $\equiv_G$ over $V(G)$ such that $v\equiv u$ if $C(v,G)= C(u,G)$. Thus, we can order the set of equivalence classes $V(G)/_{\equiv_G}=\{c_1,...,c_m\}$ such that for every $i<j$ where $c_i = [v]_{\equiv_G}$ and $c_j = [u]_{\equiv_G}$ then $C(v,G)< C(u, G)$. Therefore, we can define $\F(v,G)$ such that if $[v]_{\equiv_G}=c_i$ then $|\F(v,G)|= i-1$. Finally, we define the filter function $f$ such that $f(i) = i+1$. $f$ is well defined because, as we said, in every connected graph $G$, every node $v$ in $V(G)$ has $|\A(v,G)|\geq |V(G)|$ but we have $|V(G)/_{\equiv_G}| \leq |V(G)|$. Finally, the fact $\rank(\subc{\F,f}) = \rank(\Ce)$ follows by definition. 
\end{comment}

==> app-sec6.tex <==
\begin{comment}
\subsection*{Proof of Proposition~\ref{pro:no-monotonic-subc-measure}}

{\color{red}
Let $\hat{G}$ be the graph $(\{v_1,v_2,v_3\},\{\{v_2,v_3\}\})$.
=======
%\subsection*{Proof of Proposition~\ref{pro:no-monotonic-subc-measure}}
%
%{\color{red}
%Let $\hat{G}$ be the graph $(\{v_1,v_2,v_3\},\{\{v_2,v_3\}\})$.
%%
%Consider the measure $\Ce$ defined as follows:
%\[
%\Ce(v,G)\ =\ \begin{cases}
%1 & G \neq \hat{G} \text{ or } (G = \hat{G} \text{ and } v=v_3)\\
%3 & G = \hat{G} \text{ and } v=v_1\\
%2 & G = \hat{G} \text{ and } v=v_2.
%\end{cases}
%\]
%We first show that $\Ce$ is a subgraph motif measure. Notice that, for every vertex $v \in \ins{V}$, $\Ce(v,G_v) = \Ce(v_3,\hat{G}) = 1$. Hence, we have only two options concerning the set of connected subgraphs assigned to the vertices of $\hat{G}$ by a subgraph family, and the filtering function, which are the following: with $G_{uv} $ being the single-edge graph $(\{u,v\},\{\{u,v\}\})$, either
%\[
%\F_1(v,\hat{G})\ =\ \begin{cases}
%\emptyset & v=v_1\\
%\{G_{v_2},G_{v_2v_3}\} & v=v_2\\
%\{G_{v_3}\} & v=v_3
%\end{cases}
%\]
%with $f_1(0)=3$, $f_1(1)=1$ and $f_1(2)=2$, or
%\[
%\F_2(v,\hat{G})\ =\ \begin{cases}
%\{G_{v_1}\} & v=v_1\\
%\{G_{v_2},G_{v_2v_3}\} & v=v_2\\
%\emptyset & v=v_3
%\end{cases}
%\]
%with $f_2(0)=1$, $f_2(1)=3$ and $f_2(2)=2$. 
%%
%Now, by extending $\F_1$ and $\F_2$ in such a way that, for $(v,G) \in \vg$ with $G \neq \hat{G}$, $\F_1(v,G) = \{G_v\}$ and $\F_2(v,G) = \emptyset$, it is clear that $\Ce = \subc{\F_1,f_1} = \subc{\F_2,f_2}$. Observe, however, that $\subc{\F_1,f_1}$ and $\subc{\F_2,f_2}$ are not monotonic, and the claim follows.
%%Now, for each $i \in \{1,2\}$, by extending $\F_i$ in a such way that assigns to every pair $(v,G) \in \vg$ with $G \neq \hat{G}$ the set $\{G_v\}$ if $i=1$, and $\emptyset$ if $i=2$, it is clear that $\Ce = \subc{\F_i,f_i}$. Observe, however, that $\subc{\F_i,f_i}$ is not monotonic, for each $i \in \{1,2\}$, and the claim follows.
%}
>>>>>>> fc067a897522a3dde64b2cddfffb6a948f4ec71e
%
%
<<<<<<< HEAD
Now, by extending $\F_1$ and $\F_2$ in such a way that, for $(v,G) \in \vg$ with $G \neq \hat{G}$, $\F_1(v,G) = \{G_v\}$ and $\F_2(v,G) = \emptyset$, it is clear that $\Ce = \subc{\F_1,f_1} = \subc{\F_2,f_2}$. Observe, however, that $\subc{\F_1,f_1}$ and $\subc{\F_2,f_2}$ are not monotonic, and the claim follows.
%Now, for each $i \in \{1,2\}$, by extending $\F_i$ in a such way that assigns to every pair $(v,G) \in \vg$ with $G \neq \hat{G}$ the set $\{G_v\}$ if $i=1$, and $\emptyset$ if $i=2$, it is clear that $\Ce = \subc{\F_i,f_i}$. Observe, however, that $\subc{\F_i,f_i}$ is not monotonic, for each $i \in \{1,2\}$, and the claim follows.
}
\end{comment}



\subsection*{Proof of Theorem~\ref{the:monotonic-characterization}}
%

$\underline{(1 \Rightarrow 2).}$  By contradiction, assume that $\Ce$ does not enjoy the monotonic bounded value property, namely there exists an integer $n\geq1$ such that $|\val{}{n}(\Ce)| > n+1 - |\bval{}{n}(\Ce)|$. 
%
By hypothesis, $\Ce$ is a monotonic subgraph motif centrality measure, and thus, there exist a subgraph family $\F$ and a monotonic filtering function $f$ such that the following holds: for every $(v,G)\in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$. 
%
By the pigeonhole principle, and the fact that $\val{}{n}(\Ce) \cap \bval{}{n}(\Ce) = \emptyset$, we can conclude that there is a value $b \in (\val{}{n}(\Ce) \cup \bval{}{n}(\Ce))$ such that the following holds: there exists a pair $(v,G) \in \vg$ with $\Ce(v,G) = b$ and $|\F(v,G)| > n$. 
%
Observe that $b \not\in\val{}{n}(\Ce)$ since this would imply that $|\F(v,G)| \leq n$, which contradicts the fact that $|\F(v,G)| > n$; therefore, $b \in \bval{}{n}(\Ce)$. This means that $b < \max\val{}{n}(\Ce)$. Therefore, for some pair $(v',G') \in \vg$, we have that $f(|\F(v',G')|) = \max\val{}{n}(\Ce) > f(|\F(v,G)|) = b$, but $|\F(v',G')| \leq |\A(v',G')| \leq n < |\F(v,G)|$. This in turn implies that $f$ is not a monotonic filtering function, which leads to a contradiction. 

\medskip


$\underline{(2 \Rightarrow 1).}$ We show that there exist a subgraph family $\F$ and a monotonic filtering function $f$ such that, for every $(v,G) \in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$.
%
We start by defining a total order $\preceq_{\Ce}$ over the set of values $\val{}{}(\Ce) = \bigcup_{i=1}^{\infty}\val{}{i}(\Ce)$.
%
For some $n\geq 1$, let $D_{n}(\Ce) = \val{}{n}(\Ce) \cup \bval{}{n}(\Ce)$. By hypothesis, $\Ce$ has the monotonic bounded value property, and thus, \[
|D_n(\Ce)|\ =\ |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)| - |\val{}{n}(\Ce) \cap \bval{}{n}(\Ce)|\ =\ |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)|\ \leq\ n+1.
\]
We proceed to show that, for every $a \in D_n(\Ce)$ and $b \in D_{n+1}(\Ce)\setminus D_{n}(\Ce)$, it holds that $a<b$. 
%
By contradiction, assume that there are $a \in D_{n}(\Ce)$ and $b \in D_{n+1}(\Ce) \setminus D_{n}(\Ce)$ such that $b < a \leq \max \val{}{n}(\Ce)$. 
%
We proceed by considering two cases:

\begin{enumerate}
	\item The first case is when $b \in \val{}{n+1}(\Ce)$. In this case, by definition, $b\in \bval{}{n}(\Ce)$. Therefore, $b \in D_{n}(\Ce)$, which contradicts the fact that $b \in D_{n+1}(\Ce) \setminus D_n(\Ce)$.
	
	\item The second case is when $b \in \bval{}{n+1}(\Ce)$. In this case, $b \in \val{}{}(\Ce) \setminus \val{}{n+1}(C)\subseteq \val{}{}(\Ce)/\val{}{n}(\Ce)$ since $\val{}{n}(\Ce) \subseteq \val{}{n+1}(\Ce)$. Since $b< \max \val{}{n}(\Ce)$, by definition, we have that $b \in \bval{}{n}(\Ce)$. Therefore, $b \in D_{n}(\Ce)$, which contradicts the fact that $b \in D_{n+1}(\Ce) \setminus D_n(\Ce)$.
\end{enumerate}

We have just seen that for every $n \geq 1$, $D_n(\Ce)$ is finite. Moreover, every value of $D_{n+1}(\Ce) \setminus D_{n}(\Ce)$ is strictly greater than every value of $D_{n}(\Ce)$. With the above two facts in place, we can easily define the desired total order $\preceq_{\Ce}$ over $\val{}{}(\Ce)$:  for each $a,b \in \val{}{}(\Ce)$, $a \preceq_{\Ce} b$ if $a < b$.
%
For notational convenience, in the rest of the proof we assume that  $\val{}{}(\Ce) = \{a_1,a_2,a_3,\ldots\}$ and $a_1 \preceq_{\Ce} a_2 \preceq_{\Ce} a_3 \preceq_{\Ce} \cdots$.


Having the total order $\preceq_{\Ce}$ over $\val{}{}(\Ce)$ in place, we can now define the desired subgraph family $\F$ and monotonic filtering function $f$.
%
For an arbitrary pair $(v,G) \in \vg$, we define $\F(v,G)$ in such a way that 
\[
\Ce(v,G) = a_i \quad \text{implies} \quad |\F(v,G)| = i-1.
\]
We proceed to show that $\F$ always exists. By contradiction, assume that there is $(v,G) \in \vg$ such that $|\A(v,G)| < i-1$ but $\Ce(v,G) = a_i$; for brevity, let $n = |\A(v,G)|$. We define the set $S_i = \{a\in D_{n}(\Ce)\mid a\leq a_i\}$. Observe that
\[
n+1\ <\ i\ =\ |S_i|\ \leq\ |D_{n}(\Ce)|\ =\ |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)|, 
\]
which contradicts the fact that $\Ce$ enjoys the monotonic bounded value property. Note that, as in the proof of Theorem~\ref{the:characterization}, $\F$ can be defined in such a way that is closed under isomorphism since, by definition, $\Ce$ is closed under isomorphism.
%
We finally define the monotonic filtering function $f : \mathbb{N} \to \val{}{}(\Ce)$ as follows: for each $i \in \mathbb{N}$,
\[
f(i)\ =\ a_{i+1}. 
\]
It is straightforward to see that, for every $(v,G) \in \vg$, $\Ce(v,G) = \subc{\F,f}(v,G)$. Thus, $\Ce$ is a monotonic subgraph motif centrality measure, and Theorem~\ref{the:monotonic-characterization} follows.




\begin{comment}
	$1. \implies 2.$
	Suppose by contradiction that $\Ce$ does not satisfy axiom~\ref{def:mbvp}. Then exists $n\geq 1$ such that $|\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)| > (n+1)$. We know by hypothesis there exists a family $\F$ and function $f$ such that $\Ce=\subc{\F,f}$. Therefore, by pigeon-hole principle plus the fact $\val{}{n}(\Ce)$ and $\bval{}{n}(\Ce)$ are disjoint, there must exists values $b$ in $\val{}{n}(\Ce)\Ceup \bval{}{n}(\Ce)$ such that for a pair $(v,G)$, $\Ce(v,G) = b$ but $|F(v,G)| > n$. Now, $b$ can not be in $\val{}{n}(\Ce)$ since this would imply $|F(v,G)| \leq n$. Therefore, $b$ is in $\bval{}{n}(\Ce)$. Which means that $b < \max\val{}{n}(\Ce) = a_{\max}$. Therefore, for some pair $(v',G')$ we have $f(|\F(v',G')|) = a_{\max} > f(|\F(v,G)|)=b$ but $|\F(v',G')| \leq |\A(v',G')| \leq n < |\F(v,G)|$ which means $f$ is not a monotonic function.
	
	$2.\implies 1.$
	In order to prove this direction we need the following lemma.
	
	\begin{lemma}
		If $\Ce$ enjoys property~\ref{def:mbvp} then we can order $\val{}{}(\Ce)=\bigcup_{n}\val{}{n}(\Ce)$ such that $\val{}{}(\Ce)= \{a_1,a_2,...\}$ and for every $i<j$ then $a_i < a_j$.
	\end{lemma}
	\begin{proof}
		For a fixed $n\geq 1$ define $D_{n}(\Ce) = \val{}{n}(\Ce) \Ceup \bval{}{n}(\Ce)$. By property~\ref{def:mbvp} we know that $|D_n(\Ce)| = |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)| - |\val{}{n}(\Ce) \Ceap \bval{}{n}(\Ce)| = |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)| \leq n+1$.
	
		We will now prove that for every $n\geq1$, for every $a$ in $D_n(\Ce)$ and for every $b$ in $D_{n+1}(\Ce)/D_{n}(\Ce)$, then $a<b$. By contradiction, suppose there exists $a$ in $D_{n}(\Ce)$ and $b$ in $D_{n+1}(\Ce)/D_{n}(\Ce)$ such that $b<a\leq \max \val{}{n}(\Ce)$. In one case, if $b$ is in $\val{}{n+1}(\Ce)$, then $b\in \bval{}{n}(\Ce)$ by definition of $\bval{}{n}(\Ce)$. Therefore, $b$ is in $D_{n}(\Ce)$ which is a contradiction since we assumed $b\in D_{n+1}(\Ce)/D_n(\Ce)$. On the other side, if $b$ is in $\bval{}{n+1}(\Ce)$, then $b\in \val{}{}(\Ce)/\val{}{n+1}(C)\subseteq \val{}{}(\Ce)/\val{}{n}(\Ce)$ since $\val{}{n}(\Ce) \subseteq \val{}{n+1}(\Ce)$. In conclusion, since $b< \max \val{}{n}(\Ce)$, by definition we have that $b$ is in $\bval{}{n}(\Ce)$ as well concluding that $b\in D_{n}(\Ce)$.
		
		Finally, we just proved that every $D_n(\Ce)$ is finite for every $n$ and its values are strictly increasing from $D_{n}(\Ce)$ to $D_{n+1}(\Ce)/D_{n}(\Ce)$. This, plus the fact that $\val{}{}(\Ce) = \Ceup_{n}D_n(\Ce)$ implies we can order $\val{}{}(\Ce)$ following the usual order in $\mathbb{R}$ and starting from $D_1(\Ce)$.
	\end{proof}

Now we know that $\val{}{}(\Ce) =\{a_1,a_2,...\}$ is increasingly ordered, we can give a family $\F$ and function $f$ such that $\Ce = \subc{\F,f}$. We define $\F(v,G)$ such that $|\F(v,G)| = i-1$ if $\Ce(v,G) = a_i$. At the same time, set $f$ such that $f(i) = a_{i+1}$. To prove $\subc{\F, f}$ is well defined, suppose by contradiction there exists $(v,G)$ such that $|\A(v,G)| < i-1$ but $\Ce(v,G) = a_i$. Set $n=|\A(v,G)| < i-1$. Thus, $n+1<i$. Define the set $S_i = \{a\in D_{n}(\Ce)\mid a\leq a_i\}$. Finally, we have that $n+1 < i = |S_i| \leq |D_{n}(\Ce)| = |\val{}{n}(\Ce)| + |\bval{}{n}(\Ce)|$ which contradicts property~\ref{def:mbvp}. To see that $f$ is a monotonic function and $\Ce=\subc{\F, f}$ is just by definition.
\end{comment}



\subsection*{Proof of Theorem~\ref{the:monotonic-characterization-ranking}}
%

$\underline{(1 \Rightarrow 2).}$
Consider a centrality measure $\Ce$ that is monotonic subgraph motif relative to the induced ranking. By definition, there are a subgraph family $\F$ and a monotonic filtering function $f$ such that $\rank(\Ce) = \rank(\subc{\F,f})$.
%
Assume, by contradiction, that $\Ce$ does not enjoy the non-uniform monotonic bounded value property, i.e., there exist a graph $G$ and an integer $n \geq 1$ such that $|\val{G}{n}(\Ce)| + |\bval{G}{n}(\Ce)| > n+1$.
%
Since $|\val{G}{n}(\Ce\langle \F,f\rangle)| = |\val{G}{n}(\Ce)|$ and $|\bval{G}{n}(\Ce\langle \F,f\rangle)| = |\bval{G}{n}(\Ce)|$, 
\[
|\val{G}{n}(\Ce\langle \F,f\rangle)|+|\bval{G}{n}(\Ce\langle \F,f\rangle)|\ >\ n+1.
\] 
This means that $\subc{\F,f}$ does not enjoy the non-uniform bounded value property. Hence, by Theorem~\ref{the:monotonic-characterization}, we get that $\subc{\F,f}$ is not a subgraph motif measure relative to the induced ranking, which leads to contradiction. Consequently, $\Ce$ enjoys the non-uniform bounded value property, as needed.	

\medskip


$\underline{(2 \Rightarrow 1).}$ We need to show that there exist a subgraph family $\F$ and a monotonic filtering function $f$ such that $\rank(\Ce)=\rank(\Ce\langle \F,f\rangle)$.
%
For a graph $G$, we define the equivalence relation $\equiv_G$ over $V(G)$, and we order the equivalence classes of $V(G)/_{\equiv_G}$ as done in the proof of Theorem~\ref{the:ranking-connected-graphs}, namely with $V(G)/_{\equiv_G} = \{C_1,\ldots,C_m\}$, we assume that, for every $i,j \in [m]$, with $C_i = [v]_{\equiv_G}$ and $C_j = [u]_{\equiv_G}$, $i<j$ implies $\Ce(v,G)< \Ce(u, G)$.
%
We then define the subgraph family $\F$ and the monotonic filtering function $f$ as in the proof of Theorem~\ref{the:ranking-connected-graphs}: for every $v \in V(G)$, $|\F(v,G)|= i-1$ if $[v]_{\equiv_G} = C_i$, and $f(i) = i+1$.
%
It is not difficult to verify that indeed $\rank(\Ce)=\rank(\Ce\langle \F,f\rangle)$. It remains to show that the subgraph family $\F$ always exists.\footnote{Note that here the argument for this statement is slightly more complex than the one given in the proof of Theorem~\ref{the:ranking-connected-graphs} for a similar statement since we do not deal only with connected graphs. Moreover, we can ensure that $\F$ is closed under isomorphism by following the idea given in proof of Theorem~\ref{the:characterization}.}
%
Assume, by contradiction, that there is a vertex $v \in V(G)$ such that $[v]_{\equiv_G
} = C_i$ and $|\A(v, G)| = n < i-1$. We can show, by case analysis, that
\[
\{\Ce(w,G)\mid \Ce(w,G)< \Ce(v,G)\}\ \subseteq\ \val{G}{n}(\Ce)\cup \bval{G}{n}(\Ce). 
\]
Indeed, if $|\A(w,G)| \leq |\A(v,G)|=n$, then $\Ce(w,G) \in \val{G}{n}(\Ce)$; otherwise, if $|\A(w,G)|>|\A(v,G)|$, then, by definition, $\Ce(w,G)\in \bval{G}{n}(\Ce)$. 
%
Therefore, we can conclude that 
\begin{eqnarray*}
n+1\ <\ i &=& |\{C_1,\ldots,C_i\}|\\
&=& |\{\Ce(w,G)\mid \Ce(w,G)\ <\ \Ce(v,G)\}|\\
&\leq& |\val{G}{n}(\Ce)\cup \bval{G}{n}(\Ce)|\\
&=& |\val{G}{n}(\Ce)|+ |\bval{G}{n}(\Ce)|,
\end{eqnarray*}
which contradicts the fact the $\Ce$ enjoys the non-uniform monotonic bounded value property, and the claim follows.



\begin{comment}
we can order the set of equivalence classes as done in the proof of Theorem~\ref{the:ranking-connected-graphs}, $V(G)/_{\equiv_G} = \{c_1,c_2,...,c_k\}$ such that for $i<j$, if $c_i = [v]_{\equiv_G}$ and $c_j = [u]_{\equiv_G}$ then $\Ce(v,G) < \Ce(u, G)$. Now, consider any family $\F(v, G)$ such that $|\F(v,G)| = i-1$ if $[v]_{\equiv_G} = c_i$ and the monotonic filter function $f(i) = i+1.$ Suppose by contradiction there is a node $v$ in $G$ such that $|\A(v, G)|=n<i-1$. Consider the fact that $\{\Ce(w,G)\mid \Ce(w,G)< \Ce(v,G)\}\subseteq \val{G}{n}(\Ce)\Ceup \bval{G}{n}(\Ce)$. This can be prove by cases. If $|\A(w,G)| \leq |\A(v,G)|=n$ then $\Ce(w,G) \in \val{G}{n}(\Ce)$. On the other hand, if $|\A(w,G)|>|\A(v,G)|$ then $\Ce(w,G)\in \bval{G}{n}$ by definition. Therefore, we have $n+1 < i =|\{c_1,...,c_i\}|=|\{\Ce(w,G)\mid \Ce(w,G)< \Ce(v,G)\}|\leq |\val{G}{n}(\Ce)\Ceup \bval{G}{n}(\Ce)| = |\val{G}{n}(\Ce)|+ |\bval{G}{n}(\Ce)|$ which contradicts the bounded property. Therefore, $\F$ and $f$ are well defined. Finally, $\rank(\Ce)=\rank(\Ce\langle \F,f\rangle)$ follows by definition.
\end{comment}



\subsection*{Proof of Theorem~\ref{the:ranking-connected-graphs-monotonic}}
%

It is enough to observe that the filtering function $f$ employed in the proof of Theorem~\ref{the:ranking-connected-graphs} is monotonic.


\begin{comment}
\subsection*{Further Results}
%

As discussed in main body of the paper (see the last paragraph of Section~\ref{sec:monotonic-functions}), we can show that the non-uniform version of the monotonic bounded value property provides a necessary condition for a centrality measure being a monotonic subgraph motif measure relative to the induced ranking. We proceed to formally show this claim. We start by introducing the non-uniform version of the monotonic bounded value property:


%We extend here section~\ref{sec:monotonic-functions} in order to better understand the induced ranking of monotonic subgraph motif measures. In first place, we define an analogous property as the one in definition~\ref{def:non-uniform-bvp}.



\begin{definition}\label{def:non-uniform-mbvp}
	A centrality measure $\Ce$ enjoys the {\em non-uniform monotonic bounded value property} if, for every integer $n>0$ and graph $G \in \gr$, $|\val{G}{n}(\Ce)| \leq n+1-|\bval{G}{n}(\Ce)|$. \hfill\markfull
\end{definition}

%As expected, we will prove that the non-uniform monotonic bounded value property is a necessary condition in order to be a monotonic subgraph measure with respect to induced ranking but not sufficient. This is stated in the following theorem.

We proceed to show that the non-uniform monotonic bounded value property is {\em not} a sufficient condition for a measure being subgraph motif relative to the induced ranking, but it leads to a necessary condition. The next result can be seen as the version of Theorem~\ref{the:characterization-ranking} when we concentrate on monotonic subgraph motif measures.


\begin{theorem}
	Consider a centrality measure $\Ce$. The following are equivalent:
	\begin{enumerate}
		\item $\Ce$ is a monotonic subgraph motif relative to induce ranking.
		
		\item $\Ce$ enjoys the non uniform monotonic bounded value property.
	\end{enumerate}
\end{theorem}

\begin{proof}
	$\underline{(1 \Rightarrow 2).}$
	Consider a centrality measure $\Ce$ that is monotonic subgraph motif relative to the induced ranking. By definition, there are a subgraph family $\F$ and a monotonic filtering function $f$ such that $\rank(\Ce) = \rank(\subc{\F,f})$.
	%
	Assume, by contradiction, that $\Ce$ does not enjoy the non-uniform monotonic bounded value property, i.e., there exist a graph $G$ and an integer $n \geq 1$ such that $|\val{G}{n}(\Ce)| + |\bval{G}{n}(\Ce)| > n+1$.
	%
	Since $|\val{G}{n}(\Ce\langle \F,f\rangle)| = |\val{G}{n}(\Ce)|$ and $|\bval{G}{n}(\Ce\langle \F,f\rangle)| = |\bval{G}{n}(\Ce)|$, 
	\[
	|\val{G}{n}(\Ce\langle \F,f\rangle)|+|\bval{G}{n}(\Ce\langle \F,f\rangle)|\ >\ n+1.
	\] 
	This means that $\subc{\F,f}$ does not enjoy the non-uniform bounded value property. Hence, by Theorem~\ref{the:monotonic-characterization}, we get that $\subc{\F,f}$ is not a subgraph motif measure relative to the induced ranking, which leads to contradiction. Consequently, $\Ce$ enjoys the non-uniform bounded value property, as needed.	
		
	\medskip
	
	\andreas{This should be discussed.}
	
	$\underline{(2 \Rightarrow 1).}$ For a fixed graph $G$ we can order the set of equivalence classes as done in the proof of Theorem~\ref{the:ranking-connected-graphs}, $V(G)/_{\equiv_G} = \{c_1,c_2,...,c_k\}$ such that for $i<j$, if $c_i = [v]_{\equiv_G}$ and $c_j = [u]_{\equiv_G}$ then $\Ce(v,G) < \Ce(u, G)$. Now, consider any family $\F(v, G)$ such that $|\F(v,G)| = i-1$ if $[v]_{\equiv_G} = c_i$ and the monotonic filter function $f(i) = i+1.$ Suppose by contradiction there is a node $v$ in $G$ such that $|\A(v, G)|=n<i-1$. Consider the fact that $\{\Ce(w,G)\mid \Ce(w,G)< \Ce(v,G)\}\subseteq \val{G}{n}(\Ce)\Ceup \bval{G}{n}(\Ce)$. This can be prove by cases. If $|\A(w,G)| \leq |\A(v,G)|=n$ then $\Ce(w,G) \in \val{G}{n}(\Ce)$. On the other hand, if $|\A(w,G)|>|\A(v,G)|$ then $\Ce(w,G)\in \bval{G}{n}$ by definition. Therefore, we have $n+1 < i =|\{c_1,...,c_i\}|=|\{\Ce(w,G)\mid \Ce(w,G)< \Ce(v,G)\}|\leq |\val{G}{n}(\Ce)\Ceup \bval{G}{n}(\Ce)| = |\val{G}{n}(\Ce)|+ |\bval{G}{n}(\Ce)|$ which contradicts the bounded property. Therefore, $\F$ and $f$ are well defined. Finally, $\rank(\Ce)=\rank(\Ce\langle \F,f\rangle)$ follows by definition.
\end{proof}



%Furthermore, the proof of Theorem~\ref{the:ranking-connected-graphs} reveals that the claim holds even for monotonic subgraph motif measures, that is, for every measure $\Ce$, $\CeonC$ is a monotonic subgraph motif measure relative to the induced ranking.

%To finish our analysis o monotonic subgraph motif measures, we state the final result regarding connected graphs.

We finally observe that the proof of Theorem~\ref{the:ranking-connected-graphs} actually shows a stronger statement, namely the claim holds even if we concentrate on monotonic subgraph motif measures:

\begin{theorem}\label{the:ranking-connected-graphs-mon}
		Consider a measure $\Ce$. It holds that $\CeonC$ is a monotonic subgraph motif measure relative to the induced ranking.
\end{theorem}

\begin{proof}
	It is enough to observe that the filtering function $f$ employed in the proof of Theorem~\ref{the:ranking-connected-graphs} is monotonic.
	%see in detail proof of theorem~\ref{the:ranking-connected-graphs} and bring out the fact that the function $f$, as defined, is a monotonic function.
\end{proof}
\end{comment}

==> app-sec7.tex <==
In this final section of the appendix, we provide formal proofs for the expressibiliy/inexpressibility results presented in Section~\ref{sec:classification} (see Tables~\ref{tab:classification} and~\ref{tab:classification-monotonic}).
%
The fact that $\stress$ and $\allsub$ are (monotonic) subgraph motif (and thus, (monotonic) subgraph motif relative to the induced ranking) has been already observed in the main body of the paper. Indeed, we have seen that 
\[
\stress\ =\ \subc{\mathsf{S},f_{\times 2}} \qquad\text{and}\qquad \allsub = \subc{\mathsf{A},\log_2},
\]
where both $f_{\times 2}$ and $\log_2$ are monotonic filtering functions.


Concerning $\closeness$, we have already shown that it is not a subgraph motif measure (see Proposition~\ref{pro:closeness}), and thus, it is not a monotonic subgraph motif measure.
%
A simple inspection of the proof of Proposition~\ref{pro:closeness}, reveals that actually $\closeness$ is not a subgraph motif measure (and thus, not a monotonic subgraph motif measure) even if we concentrate on trees, as claimed in Tables~\ref{tab:classification} and~\ref{tab:classification-monotonic}.
%
The fact that $\closeness$ is not a subgraph motif measure (and thus, not a monotonic subgraph motif measure) relative to the induced ranking has been established by Proposition~\ref{pro:closeness-ranking}.




Finally, the fact that every centrality measure considered in the classification of Section~\ref{sec:classification} is (monotonic) subgraph motif relative to the induced ranking if we concentrate on connected graphs, is a consequence of Theorems~\ref{the:ranking-connected-graphs} and~\ref{the:ranking-connected-graphs-monotonic}.
%
We proceed to establish the claims stated in Tables~\ref{tab:classification} and~\ref{tab:classification-monotonic}, but are not covered by the above discussion.



\subsection*{Degree}
%

The degree centrality measure is one of the simplest measures that can be found in the literature. It states that the bigger the neighborhood of a vertex, the most central it is. Formally, given a graph $G$ and $v \in V(G)$, the {\em degree centrality} of $v$ in $G$ is
\[
\degree(v,G)\ =\ |N_G(v)|.
\]
%For every graph $G$ and node $v$ in $V(G)$, the degree centrality of $v$ in $G$ is $$\degree(v,G) = |N_G(v)|.$$
%$\degree$ essentially assign more importance to a vertex when it is connected to more nodes in the graph.
We proceed to show the following result:

\begin{proposition}\label{pro:degree}
	$\degree$ is a monotonic subgraph motif measure.
\end{proposition}

\begin{proof}
	For the degree centrality, the important subgraphs for a vertex $v$ in a graph $G$ are simply the edges of the form $\{u,v\}$.
	%
	Formally, we define the subgraph family $\F_{\degree}$ in such a way that, for every $(v,G) \in \vg$,
	\[
	\F_{\degree}(v,G)\ =\ \{(\{u,v\},\{\{u,v\}\})\mid \{u,v\}\in E(G)\}.
	\]	
	We also consider the filtering function $\mi{id}$ that is the identity over $\mathbb{N}$, i.e., $\mi{id}(x) = x$, which is monotonic.
	%
	Clearly,
	\[
	\degree(v,G)\ =\ \mi{id}(|\F_{\degree}(v,G)|)
	\]
	which in turn implies that
	\[
	\degree\ =\ \subc{\F_{\degree},\mi{id}}
	\]
	and the claim follows.
	\begin{comment}
	We can just give a family $\F$ and function $f$ such that $\degree(v,G) = \subc{\F,f}$ for every $(v,G)$. Define $\F_{\degree}(v,G) = \{(\{u,v\},\{\{u,v\}\})\mid \{u,v\}\in E(G)\}$, the important subgraphs for $v$ in $G$ are simply the edges of the form $\{u,v\}$. Finally, note that the filtering function is the identity function $\mi{id}(x) = x$. it is straightforward to see that
	$$
	\degree(v,G)\ =\ \mi{id}(|\F_{\degree}|)$$
	\end{comment}
\end{proof}


\subsection*{Cross-Clique}
%

The cross-clique centrality measure~\cite{everett1998analyzing}, was introduced in the context of analyzing virus and information propagation. It is defined as the amount of cliques containing a certain vertex. 
%
Given a graph $G$ and a vertex $ \in V(G)$, we define the set $\mi{Cl}(v,G) = \{S\in \A(v,G)\mid S \text{ is a clique}\}$. The {\em cross-clique centrality} of $v$ in $G$ is
\[
\clique(v,G)\ =\ |\mi{Cl}(v,G)|.
\]
It is straightforward to see that the following holds:


\begin{proposition}\label{pro:clique}
	$\clique$ is a monotonic subgraph motif measure.
\end{proposition}



\begin{comment}

%
We proceed to show the following:



\begin{proposition}\label{pro:decay}
	For each $\alpha\in(0,1)$, 
	\begin{enumerate}
		\item $\alpha\text{\rm -}\decay$ is not a subgraph motif measure, even if we focus on trees.
		\item $\alpha\text{\rm -}\decay$ is not a subgraph motif measure relative to the induced ranking.
	\end{enumerate}
\end{proposition}

\begin{proof}
	\underline{Item (1).} We follow the same strategy as in the proof of Proposition~\ref{pro:closeness}.
	%
	For every $n > 1$ and $i \leq n$, we have that $|\A(1, L_i)|\leq n$. Moreover, for each $\alpha\in(0,1)$, it holds that 
	\[
	\alpha\text{\rm -}\decay(1,L_i)\ =\ \sum_{j=1}^{i-1}\alpha^j \cdot |N^{j}(1,L_1)|\ =\ \sum_{j=1}^{i-1}\alpha^j\ =\ \displaystyle\frac{\alpha^{i}- \alpha}{\alpha - 1}.
	\] 
	We proceed to show that, for $n>1$ and $i,j \in\{1,...,n\}$, $i \neq j$ implies $	\alpha\text{\rm -}\decay(1,L_i) \neq 	\alpha\text{\rm -}\decay(1,L_j)$.
	%
	It is easy to see that $\alpha\text{\rm -}\decay(1,L_{i+1}) = \alpha\text{\rm -}\decay(1,L_{i}) + \alpha^{i}$. Since $\alpha^i\not= 0$, we can conclude that $\alpha\text{\rm -}\decay(1,L_{i+1}) \not= \alpha\text{\rm -}\decay(1,L_{i})$.
	%
	Moreover, this proves that if $i<j$, then $\alpha\text{\rm -}\decay(1,L_{i}) < \alpha\text{\rm -}\decay(1,L_{j})$. Now, we have that $|\val{}{6}(\alpha\text{\rm -}\decay)|\geq 6$. Similarly to what we did with $\closeness$, let us compute the centrality values for $(v, S_3)$,$(2, L_{4})$ and $(2, L_3)$. We have that
	\[
	\alpha\text{\rm -}\decay(v, S_3) = \alpha(2\alpha + 1) \qquad \alpha\text{\rm -}\decay(2, L_4) = \alpha(2+\alpha) \qquad \alpha\text{\rm -}\decay(2, L_3) = 2\alpha. 
	\]
	It is now not difficult to verify that, for every $\alpha\in(0,1)$, $|\val{}{6}(\alpha\text{\rm -}\decay)|>7$, which in turn implies that $\alpha\text{\rm -}\decay$ does not enjoy the bounded value property. Thus, by Theorem~\ref{the:characterization}, we conclude that $\alpha\text{\rm -}\decay$ is not a subgraph motif measure. This hold even if we concentrate on trees since the line and star graphs used above are trees.
	
	\medskip
	
	\underline{Item (2).} By Theorem~\ref{the:characterization-ranking}, it suffices to show that $\alpha\text{\rm -}\decay$ does not enjoy the non-uniform bounded value property.
	%
	To this end, we follow the same idea as in the proof of Proposition~\ref{pro:closeness-ranking} to, roughly speaking, gather all the graphs employed above to prove that $|\val{}{6}(\alpha\text{\rm -}\decay)|>7$ in one disconnected graph $G$. Then, by exploiting the fact that, for each $\alpha \in (0,1)$, $\alpha\text{\rm -}\decay$ is closed under isomorphism (see Definition~\ref{def:closed-under-iso}) and local (see Definition~\ref{def:locality}), we can show that $|\val{G}{6}(\alpha\text{\rm -}\decay)| > 7$.
\end{proof}
\end{comment}

\begin{comment}
Decay is another centrality measure that relies on based on the idea of distances. For a graph $G$ and node $v$ in $V(G)$, define the $i$th neighbourhood of $v$ in $G$ as the set $N^{i}_{G}(v) = \{u\in V(G)\mid d_G(v,u) = i\}$. For $\alpha\in(0,1)$, we define $\alpha-\decay$ centrality of a node $v$ in $G$ as $$\decay_{\alpha}(v,G) = \displaystyle\sum_{i = 1}^{|V(G)|}\alpha^{i}|N^{i}_{G}(v)|.$$

In essence, $\decay$ is an extended version of $\degree$ since we are giving importance to neighbourhoods beyond distance $1$ from $v$. 
Now, for each $\alpha$ we have different values for $\decay_{\alpha}$. This is the reason we say $\alpha-\decay$ is a family of centrality measures. Now, we can prove that $\alpha-\decay$ is not a subgraph motif measure for every $\alpha\in(0,1)$.

\begin{lemma}\label{lemma:ClosenotSCM}
	$\decay_\alpha$ is not a subgraph motifs centrality for every $\alpha\in(0,1)$ even relative to induced ranking.
\end{lemma}
\begin{proof}
	We use the same strategy as in proposition~\ref{pro:closeness}. Fix $n > 1$, then for every $i \leq n$ we have that $|\A(1, L_i)|\leq n$. At the same time, for $\alpha\in(0,1)$, $\decay_{\alpha}(1,L_i) = \sum_{j=1}^{i-1}\alpha^j|N^{j}(1,L_1)|=\sum_{j=1}^{i-1}\alpha^j = \displaystyle\frac{\alpha^{i}- \alpha}{\alpha - 1}$. In first place, if for a fixed $n$, we just will prove that for $i,j \in\{1,...,n\}$ such that $i\not = j$ then $\decay_{\alpha}(1,L_i)\not= \decay_{\alpha}(1,L_j)$. It is easy to see that $\decay_{\alpha}(1,L_{i+1}) = \decay_{\alpha}(1,L_{i}) + \alpha^{i}$. Since $\alpha^i\not= 0$ we can conclude that $\decay_{\alpha}(1,L_{i+1}) \not= \textsc{Decay}_{\alpha}(1,L_{i})$. More over, this proves that if $i<j$ then $\decay_{\alpha}(1,L_{i}) < \decay_{\alpha}(1,L_{j})$. Now, we have that $|\val{}{6}(\decay_{\alpha}|\geq 6$. Just as we did with closeness centrality, let's compute the values for $(v, S_3)$,$(2, L_{4})$ and $(2, L_3)$. We have that $\decay_{\alpha}(v, S_3) = \alpha(2\alpha + 1)$, $\decay_{\alpha}(2, L_4) = \alpha(2+\alpha)$ and $\decay_{\alpha}(2, L_3) = 2\alpha$. The reader can corroborate that for every $\alpha\in(0,1)$ then $|\val{}{6}(\decay_{\alpha})|>7$ which means that $\decay_{\alpha}$ does not enjoy the bounded value property.
	
	In order to prove that $\decay$ does not satisfy the non uniform property we just have to gather all the graphs we used to prove that $|\val{}{6}(\decay_{\alpha})|>7$ in one unconnected graph $G$. Thus, it is straightforward that $|\val{G}{6}(\decay_{\alpha}| > 7$.
\end{proof}
\end{comment}


\subsection*{Harmonic}
%



This centrality measure is commonly considered as an extension of $\closeness$ to disconnected graphs. 
%
Given a graph $G$ and a vertex $v \in V(G)$, the {\em harmonic centrality}~\cite{rochat2009closeness} of $v$ in $G$ is defines as
\[
\harmonic(v,G)\ =\ \begin{cases}
0 & v \text{ is isolated in } G\\
&\\
\displaystyle\sum_{u \in V(G) \setminus \{v\}}\frac{1}{d_{G}(v,u)} & \text{otherwise}.
\end{cases}
\]
%\[
%\harmonic(v,G)\ =\ \displaystyle\sum_{u \in V(G) \setminus \{v\}}\frac{1}{d_{G}(v,u)}.
%\]
Recall that, for two nodes $v,u \in V(G)$, if there is no path between them, then $d_{G}(v,u) = \infty$. Therefore, a vertex $u \in V(G)$ that is not connected with $v$ in $G$ via a path, has no impact on the harmonic centrality of $v$ in $G$. 
%
Just as $\closeness$, $\harmonic$ is usually called a geometrical measure since it relies on the distance  inside a graph. 
%Nevertheless, the standard distance is usually how $\harmonic$ is defined. 
%By convention, the harmonic centrality $\harmonic$ of an isolated vertex is equal to $0$.
We proceed to show the following:



\begin{proposition}\label{pro:harmonic}
	The following hold:
	
	\begin{enumerate}
		\item $\harmonic$ is not a subgraph motif measure, even if we focus on trees.
		\item $\harmonic$ is not a subgraph motif measure relative to the induced ranking.
	\end{enumerate}
\end{proposition}

\begin{proof}	
\underline{Item (1).} We follow the same strategy as in the proof of Proposition~\ref{pro:closeness}.
%
We first observe that $\harmonic(1,L_i) = \sum_{j=1}^{i-1}\displaystyle\frac{1}{j}$. Therefore, for $n > 1$, we have that $\harmonic(1,L_{n+1}) = \harmonic(1,L_n) + \displaystyle\frac{1}{n}$. This means $\harmonic(1,L_i)\not=\harmonic(1,L_j)$ for every $i,j$ with $i \neq j$. Hence, $|\val{}{n}(\harmonic)| \geq n-1$. Since $\harmonic(1,L_1) = 0$, we get that $|\val{}{n}(\harmonic)| \geq n$. 
%
Now, let $n = 5$. There are two pairs left: $(2, L_3)$ and $(1, S_3)$. We first observe that, for every $n > 0$,
\[
\harmonic(2, L_3)\ =\ 2\ >\ \sum_{i=1}^{n-1}\displaystyle\frac{1}{i}\ =\ \harmonic(1, L_n).
\]
Moreover, we have that
\[
\harmonic(1, S_3)\ =\ 1 + \frac{1}{2} + \frac{1}{2}\ =\ 2. 
\]
Therefore, $|\val{}{5}(\harmonic)| = 6$, which means $\harmonic$ does not violate the bounded value property for $n = 5$. However, for $n = 6$ we get that $|\val{}{6}(\harmonic)| \geq 7$ since, by definition, $\val{}{5}(\harmonic) \subseteq \val{}{6}(\harmonic)$. Now, for the pair $(2, L_4)$ we have $|\A(2, L_4)|=6$, whereas $\harmonic(2, L_4) = 2.5$. Therefore, $|\val{}{6}(\harmonic)| > 7$. Hence, $\harmonic$ violates the bounded value property. Thus, by Theorem~\ref{the:characterization}, we conclude that $\harmonic$ is not a subgraph motif measure. This hold even if we concentrate on trees since the line and star graphs used above are trees.

\medskip

\underline{Item (2).} By Theorem~\ref{the:characterization-ranking}, it suffices to show that $\harmonic$ does not enjoy the non-uniform bounded value property.
%
To this end, we follow the same idea as in the proof of Proposition~\ref{pro:closeness-ranking} to, roughly speaking, gather all the graphs employed above to prove that $|\val{}{6}(\harmonic)|>7$ in one disconnected graph $G$. Then, by exploiting the fact that $\harmonic$ is closed under isomorphism (see Definition~\ref{def:centrality-measure}) and local (see Definition~\ref{def:locality}), we can show that $|\val{G}{6}(\harmonic)| > 7$.
\end{proof}

\begin{comment}
$\harmonic$ is commonly known as an extension of $\closeness$ to unconnected graphs. We define harmonic centrality of a node $v$ in $G$ as $$\harmonic(v,G) = \displaystyle\sum_{u\not= v}\frac{1}{d_{G}(v,u)}.$$
Now, if two nodes $u$ and $v$ are not connected in $G$, we define the distance between them as $d_{G}(v,u)  = \infty$. Therefore, their interaction has no impact in the harmonic centrality of neither of them. Just as $\closeness$, $\harmonic$ is a geometrical measure. This means that depending on the definition of distance this measure can change. Nevertheless, the standard distance is usually how $\harmonic$ is defined. In this work, we assume that $\harmonic$ of an isolated vertex is equal to $0$.

\begin{lemma}\label{lemma:harmonicnot}
	$\harmonic$ is not a subgraph motif measure relative to the induced ranking even for trees.
\end{lemma}
\begin{proof}
	
	As we did for closeness centrality. We first look for the value $\harmonic(1,L_i) = \sum_{j=1}^{i-1}\displaystyle\frac{1}{j}$. Therefore, for $n > 1$, we have that $\harmonic(1,L_{n+1}) = \harmonic(1,L_n) + \displaystyle\frac{1}{n}$. Which means that for $i\not=j$ then $\harmonic(1,L_i)\not=\harmonic(1,L_j)$. Therefore, $|\val{}{n}(\harmonic)| \geq n-1$. Including the fact that $\harmonic(1,L_1) = 0$ we have that  $|\val{}{n}(\harmonic)| \geq n$. Now we fix $n = 5$. Then, there are just two pairs left, $(2, L_3)$ and $(1, S_3)$. First, we have that $\harmonic(2, L_3) = 1 + 1 = 2 > \sum_{i=1}^{n-1}\displaystyle\frac{1}{i} = \harmonic(1, L_n)$ for every $n \in \mathbb{N}$. In second place, we have that $\harmonic(1, S_3) = 1 + 1/2 + 1/2 =2$. Therefore $|\val{}{5}(\harmonic)| = 6$ which means $\harmonic$ does not violate the bounded value property for $n = 5$. However, for $n = 6$ we already know that $|\val{}{6}(\harmonic)| \geq 7$ because $\val{}{5}(C) \subseteq \val{}{6}(C)$ for every measure $C$. Now, for the pair $(2, L_4)$ we have $|\A(2, L_4)|=6$ while  $\harmonic(2, L_4) = 2.5$. Therefore, $|\val{}{6}(\harmonic)|\geq 8$ which violates the bounded value property. 
	
	Finally, for the case of the non uniform property we just have to gather every connected component in the previous proof into one big graph $G$ with all the values of centrality we already computed. Because $\harmonic$ just depends on the connected component of each node and it is a close under isomorphism measure, this concludes the proof.	
\end{proof}
\end{comment}



\subsection*{PageRank}
%


This measure, introduced in~\cite{page1999pagerank}, is used in Google's web searching engine. 
%
Given a graph $G$ with $V(G)= \{v_1,\ldots,v_{|V(G)|}\}$, we define the adjacency matrix of $G$ as the matrix $A_{G}$ such that ${A_{G}}_{ij}=1$ if $\{v_i,v_j\}\in E(G)$. 
%
We then define $\textbf{P}$ as the column-stochastic matrix with
\[
\textbf{P}_{ij}\ =\ \displaystyle\frac{{A_{G}}_{ij}}{|N_G(i)|}.
\]
In other words, $\textbf{P}$ contains the probabilities of jumping from node $i$ to node $j$ during a random walk over $G$. Let $\mathbf{v}$ be a stochastic vector $(\mathbf{1}^T\mathbf{v} = 1)$, and let $0 < \alpha < 1$ be a teleportation parameter. Then, the {\em ($\mathbf{v},\alpha$)-PageRank vector} is defined as the vector $x_{\mathbf{v},\alpha}$ that solves the equation $(I-\alpha \textbf{P})x = (1-\alpha)\mathbf{v}$. 
%
Now, given a graph $G$ with $V(G)= \{v_1,\ldots,v_{|V(G)|}\}$, the {\em PageRank centrality} of $v_i$ in $G$ is defined as
\[
\pagerank(v_i,G) = x_{0.8,\mathbf{u}}[i],
\]
where $\mathbf{u} = \mathbf{1} \cdot \frac{1}{|V(G)|}$.
%
Several variations of $\pagerank$ have been proposed in the literature. In particular, if we do not force $x_{0.8,\mathbf{u}}$ to be a probability distribution, we can ask that the sum of centrality values inside a connected component is equal to the number of nodes in that component. Therefore, this give rise to the local version of $\pagerank$, denoted $\mathsf{LPR}$. We call it local since the values in a connected component are the same regardless of the graph.


\begin{proposition}\label{pro:pagerank}
	The following hold:
	
	\begin{enumerate}
		\item $\pagerank$ is not a subgraph motif measure, even if we focus on trees.
		\item $\pagerank$ is not a subgraph motif measure relative to the induced ranking.
	\end{enumerate}
\end{proposition}

\begin{proof}
	It suffices to consider the local version of $\pagerank$ since $\rank(\pagerank) = \rank({\mathsf{LPR}})$.
	
	\medskip
	
	\underline{Item (1).}
	It can verified that $\val{L_2}{6}(\mathsf{LPR}) = \{1\}$, $\val{L_3}{6}(\mathsf{LPR}) = \{0.5, 0.33\}$, $\val{L_4}{6}(\mathsf{LPR}) = \{0.17, 0.25\}$, $\val{L_5}{6}(\mathsf{LPR}) = \{0.1\}$, $\val{L_6}{6}(\mathsf{LPR}) = \{0.07\} $, and $\val{S_3}{6}(\mathsf{LPR})=\{0.2\}$. 
	%
	Therefore,
	\[
	\{1, 0.5, 0.33, 0.17, 0.25, 0.1, 0.07, 0.2\}\ \subseteq\ \val{}{6}(\mathsf{LPR}).
	\]
	Thus, $|\val{}{6}(\mathsf{LPR})| > 7$, which implies that $\mathsf{LPR}$ does not enjoy the bounded value property. Hence, by Theorem~\ref{the:characterization}, we conclude that $\mathsf{LPR}$ is not a subgraph motif measure. This holds even if we focus on trees since the line graphs considered above are trees.
	
		
	\medskip
	
	\underline{Item (2).} By Theorem~\ref{the:characterization-ranking}, it suffices to show that $\mathsf{LPR}$ does not enjoy the non-uniform bounded value property.
	%
	To this end, we follow the same idea as in the proof of Proposition~\ref{pro:closeness-ranking} to, roughly speaking, gather all the graphs employed above to prove that $|\val{}{6}(\mathsf{LPR})|>7$ in one disconnected graph $G$. Then, by exploiting the fact that $\mathsf{LPR}$ is closed under isomorphism (see Definition~\ref{def:centrality-measure}) and local (see Definition~\ref{def:locality}), we can show that $|\val{G}{6}(\mathsf{LPR})| > 7$.
\end{proof}

\begin{comment}
This measure, introduced in~\Ceite{page1999pagerank}, is used in Google's web searching engine. 
%
For a graph $G$, define $\textbf{P}$ as the column-stochastic matrix such that $\textbf{P}_{ij} = \displaystyle\frac{A_{ij}}{|N_G(i)|}$. In other words, $\textbf{P}$ contains the probabilities of jumping from node $i$ to node $j$ during a random walk over $G$. Let $\textbf{v}$ be an stochastic vector $(e^Tv = 1)$, and let $0 < \alpha < 1$ be a teleportation parameter. Then, $\pagerank$ is defined as the vector $x$ that solves the equation $(I-\alpha P)x = (1-\alpha)v$. Finally, we define PageRank centrality as $$\pagerank_{\alpha,\textbf{v}}(v_i,G) = x_{i}.$$

Some variations of $\pagerank$ have been proposed. In particular, if we do not force $x$ to be a probability distribution, we can ask that the sum of centrality values inside a connected component is equal to the number of nodes in that component. Therefore, this give rise to a centrality measure $\textsc{LPR}$ which we will call local PageRank because the values in a connected component are always the same regardless of the graph.

\begin{lemma}
	$\text{PageRank}$ is not subgraph motif measure respect to induced ranking.
\end{lemma}

\begin{proof}
	In first place we will look at local PageRank $\textsc{LPR}$. We can compute $A_5(\textsc{LPR}) = \{3.44, 3.57, 3.89, 5, 1, 7.22, 3.52\}$ and therefore $|A_{5}(\textsc{LPR})| > 6$ which means that $\textsc{LPR}$ is not a subgraph motif measure. On the other hand, since $\textsc{LPR}$ is local and close under isomorphism, we have that $\textsc{LPR}$ is not a non subgraph motif measure respect to induced ranking. 
	
	Now, we know that $\rank({\textsc{LPR}}) = \rank(\pagerank)$. This means there can not exists $\subc{\F,f}$ such that $\rank(\pagerank) = \rank(\subc{\F,f})$.
\end{proof}
\end{comment}


\subsection*{Eigenvector}
%


Given a graph $G$ with $V(G)= \{u_1,...,u_{|V(G)|}\}$, we define the adjacency matrix of $G$ as the matrix $A_{G}$ such that ${A_{G}}_{ij}=1$ if $\{u_i,u_j\}\in E(G)$. 
Let $\lambda_{\max}(G)$ be the greatest eigenvalue of $A_G$.
%
We define the unique $L^2$ normalized eigenvector associated with $\lambda_{\max}(G)$ as $\mathbf{v}_{\max}$.
%
The {\em eigenvector centrality}~\cite{bonacich1987power} of $u_i$ in $G$ is the $i$-th entrance of $\mathbf{v}_{\max}$:
\[
\eigenvector(u_i,G)\ = \mathbf{v}_{\max}^{i}.
\]
We proceed to show the following:



\begin{proposition}\label{pro:eigenvector}
	$\eigenvector$ is not a subgraph motif measure, even if we focus on trees.
\end{proposition}

\begin{proof}
The power method is the usual way to compute $\eigenvector$~\cite{hagberg2008exploring}. With an initial vector $\mathbf{v} = \mathbf{1}$, a tolerance factor $\epsilon = 1.0e-6$, and precision of three decimals, we get the values
\begin{eqnarray*}
\val{L_3}{7}(\eigenvector) &=& \{0.5, 0.707\}\\ \val{L_4}{7}(\eigenvector) &=& \{0.371, 0.601\}\\ \val{L_5}{7}(\eigenvector) &=& \{0.288\}\\
\val{L_6}{7}(\eigenvector) &=& \{0.231\}\\ \val{L_7}{7}(\eigenvector) &=& \{0.191\}\\
\val{S_3}{7}(\eigenvector) &=& \{0.408\}
\end{eqnarray*}
and, for $T= (\{1,2,3,4,5\},\{\{1,2\},\{2,3\},\{3,4\},\{2,5\}\})$,
\[
\val{T}{7}(\eigenvector) = \{0.353\}.
\] 
Therefore, $\eigenvector$ does not enjoy the bounded value property, and thus, by Theorem~\ref{the:characterization}, it is not a subgraph motif measure. This holds even for trees since all the graphs used above are indeed trees.
\end{proof}

%\begin{proof}
%	We first prove the following: given a disconnected graph $G$ with $n = |\Ceomp(G)|$, for each component $S$ of the set $M = \{S \in \Ceomp(G)\mid \lambda_{\max}(G[V(S)]) = \lambda_{\max}(G)\}$, we have that
%	$
%	|\{\eigenvector(v,G)\mid v \in S\}| =  |\val{G[V(S)]}{}(\eigenvector)|.
%	$ 
%	%
%	In other words, each component with the same maximum eigenvalue as $G$ will have the same amount of values as the component seen as a connected graph. On the other hand, we know that $\eigenvector$ must be a unitary vector. Therefore, if $G$ has multiples connected components with the maximum eigenvalue $\lambda_{\max}$, in order to give values to every vertex in those components, the vector is forced to give different values than those given to the component seen as a connected graph. 
%	
%	Given a graph $G$, we can order its vertices $V(G) = \{v_1,\ldots,v_n\}$ in such way that, if $\Ceomp(G) = \{S_1,\ldots,S_k\}$, then, for every $m \in \{1,\ldots,k\}$, there exists $I_m=\{i_m, i_m +1, i_m+2,\ldots,i_m +|S_m|-1\}\subseteq \{1,\ldots,n\}$ such that $\{v_{s}\}_{s\in I_m} = S_m$. 
%	%
%	Therefore, the rows and columns of the adjacency matrix of $G$, $A_G$, are ordered such that there are square sections in the diagonal in $A_G$ where the $i$-th square section is the adjacency matrix of $G[V(S_i)]$, $A_{G[V(S_i)]}$. Out of these square sections the matrix $A_{G}$ just have values $0$ since vertices in different components have no connections between them. 
%	%
%	Now, for each $S_m \in M$, we know that if $b_m^{\max}$ is the eigenvector associated with $\lambda_{\max}$ in $G[V(S_m)]$, then the vector $v_{m}^{\star} = (0,0,\ldots,b_m^{\max}(1),\ldots,b_m^{\max}(|S_{m}|),0,\ldots,0)$ is a an eigenvector with eigenvalue $\lambda_{\max}$ for $A_G$ such that $v_m^{\star}(i_m+j)=b_m^{\max}(j-1)$ for $j\in\{0,\ldots,|S_m|-1\}$. This implies that any lineal combination of the vectors $v_m^{\star}$ will by an eigenvector for $A_G$ with eigenvalue $\lambda_{\max}$. Finally, we have that the unique vector $v^{\star} = c_1v_{1}^{\star} + c_2v_{2}+\ldots+v_{|M|}^{\star}$ such that $\|v^{\star}\|=1$ is the eigenvector for $\eigenvector$ centrality in $G$. In other words, for each node $v_i\in V(G)$, then $\eigenvector(v,G) = v^{\star}(i)$. As we showed, the vector $v^{\star}$ assign values for every connected component $S_m\in M$ which are proportional to $b_m^{\max}$. Therefore, we can conclude that for every $n$, $|\val{G}{n}(\eigenvector)| \geq  |\bigcup_{S\in M}\val{G[V(S)]}{n}(\eigenvector)|$.
%	%
%	Now, we will construct a sequence of graphs $G_i$ in order to prove that $|\val{}{2}(\eigenvector)| > 3$. Define the graph $G_i = (\{0,1,\ldots,i\}, \{\{i,i+1\}\mid i\mod2 = 0\})$. For $i\geq2$, we have that $G_i$ contains $i/2$ connected components. Each one is isomorphic to the line with two nodes $L_2$. Since the line with two nodes has maximum eigenvalue $\lambda_{\max} = 1$ the eigenvector $v^{\star} = (1/\sqrt{i},1/\sqrt{i},\ldots,1/\sqrt{i})$ is the eigenvector centrality vector for $G_i$. This fact implies that $|\val{}{2}(\eigenvector)| \geq |\bigcup_{j=1}^{i}\val{G_i}{n}(\eigenvector)| = i $. In other words, the set $\val{}{2}(\eigenvector)$ has infinitely many values which contradicts the bounded value property.
%	%
%	Thus, by Theorem~\ref{the:characterization}, we conclude that $\eigenvector$ is not a subgraph motif measure, even if we focus on trees.
%\end{proof}


By Theorem~\ref{the:ranking-connected-graphs-monotonic}, $\eigenvector$ is a subgraph motif measure relative to the induced ranking over connected graphs. We proceed to strengthen this result by showing that it holds over a broader class of graphs than the class of connected graphs. Let
\begin{multline*}
\mathbf{K}_1\ =\ \{G \in \mathbf{G} \mid \text{for every } G_1,G_2 \in \comp(G),\\ \lambda_{\max}(G[V(G_1)]) =\lambda_{\max}(G[V(G_2)])=\lambda_{\max}(G) \text{ implies } G_1 \cong G_2\}.
\end{multline*}
It is easy to verify that every connected graph belongs to $\mathbf{K}_1$, and that $\mathbf{K}_1$ may contain disconnected graphs. We show that:


\begin{proposition}\label{pro:eigenvector-ranking}
	$\eigenvector$ is a subgraph motif measure relative to the induced ranking when restricted to $\mathbf{K_1}$.
\end{proposition}


\begin{proof}
	From the proof of Proposition~\ref{pro:eigenvector}, we know that for every component of $M(G) = \{S\in \comp(G)\mid \lambda_{\max}(G[V(S)]) = \lambda_{\max}(G)\}$, the eigenvector centrality assigns the same amount of values to the connected component as it seen as a connected graph. On the other hand, if $S\not\in M(G)$, then, for every vertex $v \in V(S)$, we have that $\eigenvector(v,G) = 0$. Note that whenever two graphs are isomorphic they have the same values in every eigenvector. Values are just permuted depending on the isomorphism you map each graph to the other. Therefore, we have that, for every graph $G \in \mathbf{K}_1$, there exists $S \in M(G)$ such that $\val{G}{n}(\eigenvector) = \val{G[V(S)]}{n}(\eigenvector)$. In other words, when $\eigenvector$ is restricted to $\mathbf{K}_1$ it behaves like $\con\eigenvector$. Hence, we can use the same subgraph family and filter function employed in the proof of Proposition~\ref{the:ranking-connected-graphs} with the addition of value $0$ for vertices outside $S$ in $M(G)$.
\end{proof}


\begin{comment}
\begin{lemma}\label{lemma:EVnotuniform}
	$\eigenvector$ is not a subgraph motif measure.
\end{lemma}

\begin{proof}
	We will start proving that if a graph $G$ is unconnected with $n = |SCC(G)|$, then for each connected component $S$ in the set $M = \{S\in SCC(G)\mid \lambda_{\max}(G[S]) = \lambda_{\max}(G)\}$ we have that $|\{\eigenvector(v,G)\mid v\in S\}| =  |\val{G[S]}{}(\eigenvector)|$. In other words, each connected component with the same maximum eigenvalue as $G$ will have the same amount of values as the component seen as a connected graph. On the other hand, we know that $\eigenvector$ must be a unitary vector. Therefore, if $G$ has multiples connected components with the maximum eigenvalue $\lambda_{\max}$, in order to give values to every vertex in those components, the vector is forced to give different values than those given to the component seen as a connected graph. 
	
	Given a graph $G$, we can order $V(G) = \{v_1,...,v_n\}$ such that if $SCC(G) = \{S_1,S_2,...,S_k\}$ then for every $m\in \{1,...,k\}$ there exists $I_m=\{i_m, i_m +1, i_m+2,...,i_m +|S_m|-1\}\subseteq \{1,...,n\}$ such that $\{v_{s}\}_{s\in I_m} = S_m$. Therefore, the rows and columns of the adjacency matrix of $G$, $A_G$, are ordered such that there are square sections in the diagonal in $A_G$ where the $i$th square section is the adjacency matrix of $G[S_i]$, $A_{G[S_i]}$. Out of these square sections the matrix $A_{G}$ just have values $0$ because nodes in different connected components have no connections between them. Now, for each $S_m$ in $M$, we know that if $b_m^{\max}$ is the eigenvector associated with $\lambda_{\max}$ in $G[S_m]$, then the vector $v_{m}^{\star} = (0,0,...,b_m^{\max}(1),...,b_m^{\max}(|S_{m}|),0,...,0)$ is a an eigenvector with eigenvalue $\lambda_{\max}$ for $A_G$ such that $v_m^{\star}(i_m+j)=b_m^{\max}(j-1)$ for $j\in\{0,...,|S_m|-1\}$. This implies that any lineal combination of the vectors $v_m^{\star}$ will by an eigenvector for $A_G$ with eigenvalue $\lambda_{\max}$. Finally, we have that the unique vector $v^{\star} = c_1v_{1}^{\star} + c_2v_{2}+...+v_{|M|}^{\star}$ such that $\|v^{\star}\|=1$ is the eigenvector for $\eigenvector$ centrality in $G$. In other words, for each node $v_i\in V(G)$, then $\eigenvector(v,G) = v^{\star}(i)$. As we showed, the vector $v^{\star}$ assign values for every connected component $S_m\in M$ which are proportional to $b_m^{\max}$. Therefore, we can conclude that for every $n$, $|\val{G}{n}(\eigenvector)| \geq  |\Ceup_{S\in M}\val{G[S]}{n}(\eigenvector)|$. Now we will construct a sequence of graph $G_i$ in order to prove that $|\val{}{2}(\eigenvector)| > 3$. Define the graph $G_i = (\{0,1,..,i\}, \{\{i,i+1\}\mid i\mod2 = 0\})$. For $i\geq2$ we have that $G_i$ contains $i/2$ connected components. Each one is isomorphic to the line with two nodes $L_2$. Since the line with two nodes has maximum eigenvalue $\lambda_{\max} = 1$ the eigenvector $v^{\star} = (1/\sqrt{i},1/\sqrt{i},...,1/\sqrt{i})$ is the eigenvector centrality vector for $G_i$. This fact implies that $|\val{}{2}(\eigenvector)| \geq |\Ceup_{j=1}^{i}\val{G_i}{n}(\eigenvector)| = i $. In other words, the set $\val{}{2}(\eigenvector)$ has infinitely many values which contradicts the bounded value property.
\end{proof}

\begin{lemma}
	
	Define the set $K_1 = \{G\in G^{\mathcal{V}}\mid \forall S_1,S_2\in SCC(G), \lambda_{\max}(G[S_1]) =\lambda_{\max}(G[S_2])=\lambda_{\max}(G)\implies S_1\Ceong S_2\}$. $\eigenvector$ centrality is in subgraph motif with respect to induced ranking when restricted to graphs in $K_1$.
\end{lemma}

\begin{proof}
	From lemma~\ref{lemma:EVnotuniform}'s proof we know that for every connected component in the set $M(G) = \{S\in SCC(G)\mid \lambda_{\max}(G[S]) = \lambda_{\max}(G)\}$ then eigenvector centrality assigns the same amount of values to the connected component as it seen as a connected graph. On the other hand, if $S\not\in M(G)$ the for every node $v$ in $S$ we have that $\eigenvector(v,G) = 0$. On the other hand, when two graphs are isomorphic they have the same values in every eigenvector. Values are just permuted depending on the isomorphism you map each graph to the other. Therefore, we have that for every $G\in K_1$ there exists $S\in M(G)$ such that $\val{G}{n}(\eigenvector) = \val{G[S]}{n}(\eigenvector)$. In other words, when $\eigenvector$ is restricted to $K_1$ it behaves like $\Ceon\eigenvector$ so we can use the same family and filter function defined in proposition~\ref{the:ranking-connected-graphs} with the addition of value $0$ for nodes outside $S$ in $M(G)$.
\end{proof}
\end{comment}


\subsection*{Betweenness}
%


This centrality measure is similar to $\stress$ with the difference that we take the proportion of shortest paths going through a certain vertex. 
%
Formally, given a graph $G$ and a vertex $v \in V(G)$, the {\em betweenness centrality}~\cite{freeman1977set} of $v$ in $G$ is
\[
\betweeness(v,G)\ =\ \sum_{(u,w)\in (K_{v}(G) \setminus \{v\})^{2}}\displaystyle\frac{|S_G^v(u,w)|}{|S_G(u,w)|}.
\]
%In some sense, betweenness centrality is based on the notion of distance. However, we do not assign importance to the distance itself but to the structures where node $v$ belongs. This measure is closely related with connectivity or flux between nodes and it is natural to ask whether it is a subgraph motif measure.
We proceed to show the following result:


\begin{proposition}\label{pro:betweenness-positive-trees}
	$\betweeness$ is a subgraph motif measure when restricted to trees.
\end{proposition}


\begin{proof}
	We need to show that there exist a subgraph family $\F$ and a filtering function $f$ such that $\betweeness = \subc{\F,f}$.
	%
	Since we focus on trees, there is natural subgraph  family that does the job. For every tree $T$ and $v \in V(T)$, we define $\F$ as follows:
	\[
	\F(v,T)\ =\ \{\pi_{uw}\in\A(v, T)\mid u,w \in V(T) \setminus \{v\} \text{ and } \pi_{uw} \in S_T(u,w)\}. 
	\]
	For the filtering function we simply use the function $f_{\times 2}$, i.e., $f_{\times 2}(x) = 2x$. 
	%
	It remains to show that, for every $v \in V(T)$, $\betweeness(v,T) = f_{\times 2}(|\F(v,T)|)$. In trees we know that, for every pair of vertices $u,v$, it holds that $|S_G(u,v)| = 1$. Therefore, for any $v\in V(T)$, we have that $\betweeness(v,T) = \stress(v, T) = f_{\times 2}(|\F(v,T)|)$, and the claim follows.
\end{proof}

One can define a broader class of graphs than the class of trees over which $\betweeness$ still a subgraph motif measure. Let
\[
\mathbf{C}_1 = \{G \in \mathbf{G} \mid \text{for every } v,u \in V(G), |S_G(v,u)| \leq 1\},
\]
i.e., it collects all the graphs such that, for every two nodes $v,u$ in $G$, there exists exactly one shortest path from $v$ to $u$, a property that trees trivially satisfy. It is then not difficult to show the following result by exploiting the subgraph family and the filtering function used in the proof of Proposition~\ref{pro:betweenness-positive-trees}:

\begin{proposition}\label{pro:betweenness-positive-c1}
		$\betweeness$ is a subgraph motif measure when restricted to $\mathbf{C}_1$.
\end{proposition}

It turned out that the question whether $\betweeness$ is a subgraph motif in general is a non-trivial one that remains open. We conclude this section by dealing with rankings. We proceed to show the following inexpressibility result:



\begin{proposition}\label{pro:betweenness}
	The following hold:
	
	\begin{enumerate}
		\item $\betweeness$ is not a monotonic subgraph motif measure, even if we focus on connected graphs.
		\item $\betweeness$ is not a monotonic subgraph motif measure relative to the induced ranking.
	\end{enumerate}
\end{proposition}

\begin{proof}
	\underline{Item (1).} We are going to show that $\betweeness$ does not enjoy the monotonic bounded value property, and thus, by Theorem~\ref{the:monotonic-characterization}, it is not a monotonic subgraph motif measure.
	%
	For $n\geq1$, consider the connected graph $H_n = (V_n, E_n)$, where
	\begin{eqnarray*}
	V_n &=& \{1,2,...,n+2\},\\
	E_n &=& \{\{1, i\} \mid i \in\{3,4,\ldots,n+2\}\}\cup\{\{2, i\}\mid i \in\{3,4,.\ldots,n+2\}\}. 
	\end{eqnarray*}
	It can be verified that $\betweeness(3, H_n) = \frac{2}{n}$. However, for $n>1$, $|\A(3, H_n)| > 4$. Therefore, we have that
	\[
	|\val{}{4}(\betweeness)| + |\bval{}{4}(\betweeness)|\ >\ 5,
	\]
	which implies that $\betweeness$ does not enjoy the monotonic bounded value property.
	
	\medskip
	
	\underline{Item(2).} By Theorem~\ref{the:characterization-ranking}, it suffices to show that $\betweeness$ does not enjoy the non-uniform bounded value property.
	%
	Since $\betweeness$ is closed under isomorphism and local, we will use the same strategy as we did in analogous proofs. In particular, we define the graph $G$ as the minimal graph with the following property: for every graph $G' \in \{H_1,H_2,\ldots,H_5, H_6\}$, there is $G''\in\comp(G)$ such that $G''$ is isomorphic to $G'$. We can then show that
	\[
	|\val{G}{4}(\betweeness)| + |\bval{G}{4}(\betweeness)|\ >\ 5,
	\]
	which implies that $\betweeness$ does not enjoy the non-uniform monotonic bounded value property, and the claim follows.
\end{proof}


\begin{comment}
$\betweeness$ centrality is similar to $\stress$ but now we take the proportion of shortest paths going through a node $v$. Formally, we define the $\betweeness$ centrality of $v$ in $G$ as $$\betweeness(v,G) = \sum_{(u,w)\in (K_{v}(G)-\{v\})^{2}}\displaystyle\frac{|S_G^v(u,w)|}{|S_G(u,w)|}.$$
In some sense, betweenness centrality is based on the notion of distance. However, we do not assign importance to the distance itself but to the structures where node $v$ belongs. This measure is closely related with connectivity or flux between nodes and it is natural to ask whether it is a subgraph motif measure.

\begin{lemma}
	$\textsc{Betweenness}$ is a subgraph motif measure over trees.
\end{lemma}
\begin{proof}
	For trees we have a very natural family of substructures that can define $\betweeness$ centrality. For every tree $T$ and node $v$ in $T$ define the family $\F(v,T) = \{\pi_{uw}\in\A(v, T)\mid \pi_{uw} \text{ is a shortest path connecting } u \text{ and }w\wedge u\not=v\wedge w\not=v\}.$ For the filter function we just need the identity $\ \mi{id}(x) =x$. Finally, we just need to prove that $|\F(v,T)|=\betweeness(v,T)$. In trees we know that for every pair of nodes $u,v$ then $|S_G(u,v)| = 1$. Therefore, for any $v\in V(T)$ we have that $\textsc{Betweenness}(v,T)=\stress(v, T) = |\F(v,T)|.$
\end{proof}
One can define a broader class of graphs $C_1$ where $\betweeness$ still a subgraph motif measure.
\begin{corollary}
	Define the set of graphs $C_1 = \{G\in \mathcal{G}^{\mathcal{V}}\mid \forall v,u\in V(G), |D_{v,u}|=1\}$, then $\betweeness$ is subgraph motif over $C_1$.
\end{corollary}
\begin{proof}
	We can use the same family and function as we did for last lemma since $|S_G(u,v)|=1$ for every $G$ in $C_1$.
\end{proof}
In order to prove that $\betweeness$ is a subgraph motif measure in general, one should prove the bounded value property. However, this task is not trivial since the bounded value property runs over every $n$. Intuitively, we can expect the difficulty of such proof by looking at the following result.
\begin{theorem}\label{th:beetnot}
	If $\betweeness$ is a subgraph motif measure, $C\langle F,f\rangle$. Then $f$ is not a monotonic function.
\end{theorem}
\begin{proof}
	We will prove this by using theorem~\ref{the:monotonic-characterization}. For $n\geq1$, define the set of nodes $V_n = \{1,2,...,n+2\}$ and the set of edges $E_n = \{\{1, i\}\mid i \in\{3,4,...,n+2\}\}\Ceup\{\{2, i\}\mid i \in\{3,4,...,n+2\}\}$. Define the graph $H_n = (V_n, E_n)$. We have that $\betweeness(3, H_n) = 2/n$. However, for $n>1$ we have that $|\A(3, H_n)| > 4$. Therefore, we have that $|\val{}{4}(\betweeness)| + |\bval{}{4}(\betweeness)| > 5$ which contradicts property~\ref{def:mbvp}.
\end{proof}

To conclude this section, we just have left to prove that betweenness centrality is not a monotonic subgraph motif measure relative to ranking as stated in table~\ref{tab:classification-monotonic}.

\begin{theorem}
$\betweeness$ is not a monotonic subgraph motif measure relative to induced ranking.
\end{theorem}

\begin{proof}
	Since $\betweeness$ satisfies the close under isomorphism and locality properties, we will use the same strategy as we did for other induced rankings. Define the graph $G$ as the minimal graph with the following property: for every graph $G' \in\{H_1,H_2,..., H_5, H_6\}$ ($H_n$ is defined in the proof of theorem~\ref{th:beetnot}) there exists a component $G''\in\Ceomp(G)$ such that $G''$ is isomorphic to $G'$. Thus, it follows from the values of $\betweeness$ that $|\val{G}{4}| + |\bval{G}{4}| > 5$ which contradicts the non uniform monotonic bounded value property.
\end{proof}
\end{comment}

==> graph-ex1.tex <==
	\newcommand{\fsize}{\normalsize}
	\begin{tikzpicture}[node distance=1.2cm] 
	\tikzset{     
		e4c node/.style={circle,draw,minimum size=0.5cm,inner sep=0}, 
		e4c edge/.style={sloped,above}
	}
	
	\node[e4c node] (v) at (0, 0) {\fsize $v_2$}; 
	
	\node[e4c node, below left of=v] (u1) {\fsize $v_1$}; 
	\node[e4c node, below right of=v] (u2) {\fsize $v_3$};
	
	
	\path[draw]
	(v) edge[e4c edge] node {}  (u1)
	;
	
	\node[node distance=0.7cm, above of=v] {\fsize $H$}; 
	\node[node distance=0.5cm, right of=v] {\color{red} $3$}; 
	\node[node distance=0.5cm, right of=u2] {\color{red} $4$}; 
	\node[node distance=0.5cm, right of=u1] {\color{red} $2$}; 

\end{tikzpicture}

==> graph-ex2.tex <==
\newcommand{\fsize}{\normalsize}
\begin{tikzpicture}[node distance=1.2cm] 
	\tikzset{     
		e4c node/.style={circle,draw,minimum size=0.5cm,inner sep=0}, 
		e4c edge/.style={sloped,above}
	}
	
	\node[e4c node] (v) at (0, 0) {\fsize $v_2$}; 
	
	\node[e4c node, below left of=v] (u1) {\fsize $v_1$}; 
	\node[e4c node, below right of=v] (u2) {\fsize $v_3$};
	\node[e4c node, right of=v] (u3) {\fsize $v_4$};
	
	
	\path[draw]
	(v) edge[e4c edge] node {}  (u1)
	;
	
	\node[node distance=0.7cm, above of=v] {\fsize $S$}; 
	\node[node distance=0.5cm, right of=v] {\color{red} $3$}; 
	\node[node distance=0.5cm, right of=u2] {\color{red} $4$}; 
	\node[node distance=0.5cm, right of=u1] {\color{red} $2$}; 
	\node[node distance=0.5cm, right of=u3] {\color{red} $5$}; 
	
\end{tikzpicture}
